Data-Driven Model Invalidation for Unknown Lipschitz Continuous Systems via Abstraction

In this paper, we consider the data-driven model invalidation problem for Lipschitz continuous systems, where instead of given mathematical models, only prior noisy sampled data of the systems are available. We show that this data-driven model invalidation problem can be solved using a tractable feasibility check. Our proposed approach consists of two main components: (i) a data-driven abstraction part that uses the noisy sampled data to over-approximate the unknown Lipschitz continuous dynamics with upper and lower functions, and (ii) an optimization-based model invalidation component that determines the incompatibility of the data-driven abstraction with a newly observed length-T output trajectory. Finally, we discuss several methods to reduce the computational complexity of the algorithm and demonstrate their effectiveness with a simulation example of swarm intent identification.

==> sec_abstraction.tex <==
%!TEX root = main.tex
\section{Affine Abstraction}

The affine abstraction defined in Problem \ref{problem1} is formulated as a robust optimization program.
Since there are nonlinear uncertainties in \eqref{p1:a}-\eqref{p1:b}, i.e., multiplication of two uncertain sets, and the semi-infinite constraints as illustrated in \eqref{p1:a}-\eqref{p1:c}, the formulation in Problem \ref{problem1} is not practically solvable.
To cope with this, we leverage the form of the uncertainties associated with the system matrices and tools from robust optimization \cite{ben2009robust, bertsimas2011theory} to convert this problem into an LP, which can be readily and efficiently solved. 

%
%\subsection{Equivalent LP via Double Robustification}
%
%Based on the definition of an interval matrix, the uncertainty system matrix $G$ determined by the interval matrix $G^I = [\underline{G}, \overline{G}]$ can be equivalently written as $n$ polytopes
%\begin{align}
% (G)_i^\mathsf{T} \in \mathcal{G}_i = \left \{ g \in \mathbb{R}^{\xi} : L g \le d_i \right \}, \forall i \in [n],
%\end{align}
%where the matrix $L\in \mathbb{R}^{2\xi \times \xi}$ and vector $d_i \in \mathbb{R}^{2\xi}$ are defined as
%\begin{align} \label{uncertainty_ineq}
%L = \begin{bmatrix} I_{\xi} \\ -I_{\xi} \end{bmatrix}, \; d_i = \begin{bmatrix} (G_{u})_i^\mathsf{T}  \\   -(G_{l})_i^\mathsf{T} \end{bmatrix} .
%\end{align}
%Consequently, the Problem \ref{problem1} with row-wise uncertainty can be rewritten as 
%\begin{subequations} 
%\begin{align} 
%\underset{\theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}} {\text{min}}  \quad & \theta  \notag \\ 
%\text{s.t.} \hspace{0.70cm} 
%& \hspace{-0.1cm} \begin{array}{l} \label{pAB_1:a}
%\left( (G)_i^\mathsf{T} \right)^\mathsf{T} {h}(k) \le  (\overline{G})_i {h}(k)  + \overline{b}_i ,   \\ \vspace{-0.1cm}
%\forall (G)_i^\mathsf{T} \in \mathcal{G}_i, \forall h(k) \in \mathcal{H},  \forall i \in [n],  
%\end{array} \\
%& \hspace{-0.1cm}  \begin{array}{l} \label{pAB_1:b}
% -\left( (G)_i^\mathsf{T} \right)^\mathsf{T} {h}(k) \le  -(\underline{G})_i {h}(k)  - \underline{b}_i ,   \\ \vspace{-0.05cm}
%\forall (G)_i^\mathsf{T} \in \mathcal{G}_i, \forall h(k) \in \mathcal{H}, \forall i \in [n],   
%\end{array} \\
%& \hspace{-0.1cm}  \max_{h(k) \in \mathcal{H}} \|\overline{f} \left( h(k) \right)- \underline{f}\left( h(k) \right) \|_\infty \le \theta . \label{pAB_1:c}
%\end{align}
%\end{subequations}
%
%Next, for each of constraints \eqref{pAB_1:a} and \eqref{pAB_1:b}, we use robust optimization approach twice (the first is with respect to uncertainty set $\mathcal{G}_i$  and the second is with respect to uncertain set $\mathcal{H}$) to make above problem solvable.
%
%Consider the constraint \eqref{pAB_1:a} that is equivalent to the following subproblem if we deal with the uncertain set $\mathcal{G}_i$ first:
%\begin{gather}
%\begin{array}{l} \label{pAB_1:aa}
%\left[  \begin{matrix}
% \underset{(G)_i^\mathsf{T} \in \mathbb{R}^{\xi}}  {\text{max}}  &  \left( (G)_i^\mathsf{T} \right)^\mathsf{T} {h}(k)  \\
%\text{s.t.}  & \hspace{-0.1cm} L  (G)_i^\mathsf{T}  \leq d_i
%\end{matrix} \right ] \le (\overline{G})_i {h}(k)  + \overline{b}_i, \\
%~ \forall h(k) \in \mathcal{H},  \forall i \in [n].
%\end{array}
%\end{gather}
%Applying the LP duality to the inner maximization subproblem in \eqref{pAB_1:aa} yields
%\begin{align}
%\begin{array}{l} \label{pAB_1:aa_dual}
%\left[  \begin{matrix}
%\underset{\overline{p}_{i} \in \mathbb{R}^{2 \xi}}  {\text{min}}  &  \hspace{-1.15cm} \overline{p}_{i}^\mathsf{T} d_i  \\
%\text{s.t.} &  L^\mathsf{T} \overline{p}_{i} = h(k) \\
%& \hspace{-0.9cm} \overline{p}_{i} \ge 0
%\end{matrix} \right ] \le (\overline{G})_i {h}(k)  + \overline{b}_i, \\
%~ \forall h(k) \in \mathcal{H},  \forall i \in [n].
%\end{array}
%\end{align}
%Let $\overline{p}_{i} =  \begin{bmatrix} \overline{p}_{i,1} \\ \overline{p}_{i,2} \end{bmatrix}$ with $ \overline{p}_{i,1} \in \mathbb{R}^{\xi}$ and $ \overline{p}_{i,2} \in \mathbb{R}^{\xi}$. 
%Based on the constraints in the minimization problem \eqref{pAB_1:aa_dual} and \eqref{uncertainty_ineq}, we have 
%\begin{align} \label{pAB_1:aa_dual_eqn}
%\overline{p}_{i,1} = \overline{p}_{i,2} + h(k). 
%\end{align}
%Then, substituting \eqref{pAB_1:aa_dual_eqn} into \eqref{pAB_1:aa_dual} eliminates $\overline{p}_{i,1}$ and yields
%\begin{align}
%\hspace{-0.25cm} \begin{array}{l} 
%\left[  \begin{matrix} \vspace{-0.05cm}
%\underset{\overline{p}_{i,2} \in \mathbb{R}^{\xi}}  {\text{min}}  &    ({G_u})_i h(k) -  \left( ({G_l})_i - ({G_u})_i \right) \overline{p}_{i,2} \\ 
%\text{s.t.} & \hspace{-2.5cm} \overline{p}_{i,2} + h(k) \ge 0 \\
%& \hspace{-3.6cm} \overline{p}_{i,2} \ge 0
%\end{matrix} \right ]  \\
%\hspace{0.1cm} \le (\overline{G})_i {h}(k)  + \overline{b}_i, \,\,\forall h(k) \in \mathcal{H},  \forall i \in [n].
%\end{array}
%\end{align}
%% Since disregarding the $\min$
%Consider $\overline{p}_{i,2}$ as a decision variable in the outer minimization, the constraint \eqref{pAB_1:a} is further equivalent to 
%\begin{subequations} 
%\begin{align} 
%& \hspace{-0.41cm}\begin{array} {l} \label{pAB_1:aa_dual_final}
%\begin{bmatrix} ({G_u})_i -  (\overline{G})_i  \\ - I_{\xi} \end{bmatrix}  {h}(k) \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \overline{p}_{i,2} +  \overline{b}_i \\ \overline{p}_{i,2}  \end{bmatrix} \hspace{-0.05cm}, \\ \vspace{-0.1cm}
%~\forall h(k) \in \mathcal{H},  \forall i \in [n],
%\end{array} \\ 
%& \hspace{-0.1cm} \overline{p}_{i,2} \ge 0,  \,\, \forall i \in [n]. \label{pAB_1:aa_dual_var}
%\end{align}
%\end{subequations} 
%Now it is ready to consider the uncertainty set $\mathcal{H}$ in constraint \eqref{pAB_1:a}.  Since its equivalence \eqref{pAB_1:aa_dual_final} can be written as 
%\begin{align}
% \begin{array}{l} 
%\left[  \begin{matrix}
% \underset{h(k) \in \mathbb{R}^{\xi}}  {\text{max}}  &  \begin{bmatrix} ({G_u})_i -  (\overline{G})_i  \\ - I_{\xi} \end{bmatrix}  {h}(k)   \\
%\text{s.t.}  & \hspace{-1.3cm} Q  h(k) \leq q
%\end{matrix} \right ] \\
%\hspace{0.1cm} \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \overline{p}_{i,2} +  \overline{b}_i \\ \overline{p}_{i,2}  \end{bmatrix}, ~  \forall i \in [n],
%\end{array}
%\end{align}
%the duality becomes
%\begin{align}
%\hspace{-0.25cm} \begin{array}{l} 
%\left[  \begin{matrix} \vspace{-0.05cm}
%\underset{\overline{\Pi}_i \in \mathbb{R}^{k \times (\xi+1)}}  {\text{min}}  &   \hspace{-2.9cm}   \overline{\Pi}_i^\mathsf{T} q \\ 
%\text{s.t.} & \overline{\Pi}_i^\mathsf{T} Q  = \begin{bmatrix} ({G_u})_i -  (\overline{G})_i  \\ - I_{\xi} \end{bmatrix}  \\
%& \hspace{-2.5cm} \overline{\Pi}_i \ge 0
%\end{matrix} \right ]  \\
%\hspace{0.1cm} \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \overline{p}_{i,2} +  \overline{b}_i \\ \overline{p}_{i,2}  \end{bmatrix}, ~  \forall i \in [n].
%\end{array}
%\end{align}
%Incorporating this dual subproblem into the original constraint and considering $\overline{\Pi}_i$ as a decision variable in the outer minimization, we convert the constraint \eqref{pAB_1:a} to the following linear constraints 
%\begin{subequations} \label{pAB_1:upper_ddual_final}
%\begin{align} 
%& \hspace{-0.41cm} \begin{array} {l} \label{pAB_1:aa_ddual_final}
%\overline{\Pi}_i^\mathsf{T} q \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \overline{p}_{i,2} +  \overline{b}_i \\ \overline{p}_{i,2}  \end{bmatrix}, ~  \forall i \in [n], \\ 
%\end{array} \\
%& \hspace{-0.41cm} \begin{array} {l}
%\overline{\Pi}_i^\mathsf{T} Q  = \begin{bmatrix} ({G_u})_i -  (\overline{G})_i  \\ - I_{\xi} \end{bmatrix} , ~  \forall i \in [n],
%\end{array} \\
%& \hspace{-0.2cm} \overline{\Pi}_i \ge 0 , ~  \forall i \in [n], \\
%& \hspace{-0.2cm} \overline{p}_{i,2} \ge 0,  \,\, \forall i \in [n]. \label{pAB_1:aa_ddual_var}
%\end{align}
%\end{subequations} 
%
%%Using the robust optimization approach again to \eqref{pAB_1:aa_dual_final}, we have
%
%Similarly, the lower hyperplane constraints in \eqref{pAB_1:b} can be rewritten as
%\begin{gather}
%\begin{array}{l} \label{pAB_1:aaa}
%\left[  \begin{matrix}
% \underset{(G)_i^\mathsf{T} \in \mathbb{R}^{\xi}}  {\text{max}}  &  -\left( (G)_i^\mathsf{T} \right)^\mathsf{T} {h}(k)  \\
%\text{s.t.}  & \hspace{-0.1cm} L  (G)_i^\mathsf{T}  \leq d_i
%\end{matrix} \right ] \le -(\underline{G})_i {h}(k)  - \underline{b}_i, \\
%~ \forall h(k) \in \mathcal{H},  \forall i \in [n].
%\end{array}
%\end{gather}
%Applying the LP duality to the inner maximization subproblem in \eqref{pAB_1:aaa} yields
%\begin{align}
%\begin{array}{l} \label{pAB_1:aaa_dual}
%\left[  \begin{matrix}
%\underset{\underline{p}_{i} \in \mathbb{R}^{2 \xi}}  {\text{min}}  &  \hspace{-1.15cm} \underline{p}_{i}^\mathsf{T} d_i  \\
%\text{s.t.} &  -L^\mathsf{T} \underline{p}_{i} = h(k) \\
%& \hspace{-0.9cm} \underline{p}_{i} \ge 0
%\end{matrix} \right ] \le -(\underline{G})_i {h}(k) - \underline{b}_i, \\
%~ \forall h(k) \in \mathcal{H},  \forall i \in [n].
%\end{array}
%\end{align}
%We further let $\underline{p}_{i} =  \begin{bmatrix} \underline{p}_{i,1} \\ \underline{p}_{i,2} \end{bmatrix}$ with $ \underline{p}_{i,1} \in \mathbb{R}^{\xi}$ and $ \underline{p}_{i,2} \in \mathbb{R}^{\xi}$. 
%Based on the constraints in the minimization problem \eqref{pAB_1:aa_dual} and \eqref{uncertainty_ineq}, we have 
%\begin{align} \label{pAB_1:aa_dual_eqn}
%\underline{p}_{i,2} = \underline{p}_{i,1} + h(k). 
%\end{align}
%Then, substituting \eqref{pAB_1:aa_dual_eqn} into \eqref{pAB_1:aa_dual} eliminates $\underline{p}_{i,2}$ and yields
%\begin{align}
%\hspace{-0.25cm} \begin{array}{l} 
%\left[  \begin{matrix} \vspace{-0.05cm}
%\underset{\underline{p}_{i,1} \in \mathbb{R}^{\xi}}  {\text{min}}  &    -({G_l})_i h(k) -  \left( ({G_l})_i - ({G_u})_i \right) \underline{p}_{i,1} \\ 
%\text{s.t.} & \hspace{-2.7cm} \underline{p}_{i,1} + h(k) \ge 0 \\
%& \hspace{-3.8cm} \underline{p}_{i,1} \ge 0
%\end{matrix} \right ]  \\
%\hspace{0.1cm} \le - (\underline{G})_i {h}(k)  - \underline{b}_i, \,\,\forall h(k) \in \mathcal{H},  \forall i \in [n].
%\end{array}
%\end{align}
%Consider $\underline{p}_{i,1}$ as a decision variable in the outer minimization, the constraint \eqref{pAB_1:b} is further equivalent to 
%\begin{subequations} 
%\begin{align} 
%& \hspace{-0.41cm}\begin{array} {l} \label{pAB_1:aaa_dual_final}
%\begin{bmatrix} (\underline{G})_i -  ({G}_l)_i  \\ - I_{\xi} \end{bmatrix}  {h}(k) \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \underline{p}_{i,1}  -  \underline{b}_i \\ \underline{p}_{i,1}  \end{bmatrix} \hspace{-0.05cm}, \\ \vspace{-0.1cm}
%~\forall h(k) \in \mathcal{H},  \forall i \in [n],
%\end{array} \\ 
%& \hspace{-0.1cm} \underline{p}_{i,1} \ge 0,  \,\, \forall i \in [n]. \label{pAB_1:aaa_dual_var}
%\end{align}
%\end{subequations} 
%Now it is ready to consider the uncertainty set $\mathcal{H}$ in constraint \eqref{pAB_1:b}.  Since its equivalence \eqref{pAB_1:aaa_dual_final} can be written as 
%\begin{align}
% \begin{array}{l} 
%\left[  \begin{matrix}
% \underset{h(k) \in \mathbb{R}^{\xi}}  {\text{max}}  &  \begin{bmatrix} (\underline{G})_i -  ({G}_l)_i \\ - I_{\xi} \end{bmatrix}  {h}(k)   \\
%\text{s.t.}  & \hspace{-1.3cm} Q  h(k) \leq q
%\end{matrix} \right ] \\
%\hspace{0.1cm} \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \underline{p}_{i,1} - \underline{b}_i \\ \underline{p}_{i,1}  \end{bmatrix}, ~  \forall i \in [n],
%\end{array}
%\end{align}
%the duality becomes
%\begin{align}
%\hspace{-0.25cm} \begin{array}{l} 
%\left[  \begin{matrix} \vspace{-0.05cm}
%\underset{\underline{\Pi}_i \in \mathbb{R}^{k \times (\xi+1)}}  {\text{min}}  &   \hspace{-2.8cm}   \underline{\Pi}_i^\mathsf{T} q \\ 
%\text{s.t.} & \underline{\Pi}_i^\mathsf{T} Q  = \begin{bmatrix} (\underline{G})_i -  ({G}_l)_i  \\ - I_{\xi} \end{bmatrix}  \\
%& \hspace{-2.4cm} \underline{\Pi}_i \ge 0
%\end{matrix} \right ]  \\
%\hspace{0.1cm} \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \underline{p}_{i,1} -  \underline{b}_i \\ 
% \underline{p}_{i,1}  \end{bmatrix}, ~  \forall i \in [n]. 
%\end{array}
%\end{align}
%Incorporating this dual subproblem into the original constraint and considering $\underline{\Pi}_i$ as a decision variable in the outer minimization, we convert the constraint \eqref{pAB_1:b} to the following linear constraints 
%\begin{subequations}  \label{pAB_1:lower_ddual_final}
%\begin{align} 
%& \hspace{-0.41cm} \begin{array} {l} \label{pAB_1:aaa_ddual_final}
%\underline{\Pi}_i^\mathsf{T} q \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \underline{p}_{i,1} - \underline{b}_i \\ \underline{p}_{i,1}  \end{bmatrix}, ~  \forall i \in [n], \\ 
%\end{array} \\
%& \hspace{-0.41cm} \begin{array} {l}
%\underline{\Pi}_i^\mathsf{T} Q  = \begin{bmatrix} (\underline{G})_i -  ({G}_l)_i  \\ - I_{\xi} \end{bmatrix} , ~  \forall i \in [n],
%\end{array} \\
%& \hspace{-0.2cm} \underline{\Pi}_i \ge 0 , ~  \forall i \in [n], \\
%& \hspace{-0.2cm} \underline{p}_{i,1} \ge 0,  \,\, \forall i \in [n]. \label{pAB_1:aaa_ddual_var}
%\end{align}
%\end{subequations} 
%Finally, for the constraint in \eqref{pAB_1:c}, due to the fact that
%\begin{align*}
% \|\overline{f} \left( h(k) \right) - \underline{f} \left( h(k) \right) \|_\infty = \max_{i \in [n]} \;( \overline{f}_i \left( h(k) \right)- \underline{f}_i \left( h(k) \right) ), 
% \end{align*}
%it can be written as
%\begin{align}
% \max_{h(k) \in \mathcal{H}} \max_{i \in [n]} \; ( \overline{f}_i \left( h(k) \right)- \underline{f}_i \left( h(k) \right) ) \le \theta ,
% \end{align}
% which further implies that 
%% \begin{align}
%% \max_{h(k) \in \mathcal{H}}  \; \overline{G} h(k) -\underline{G} h(k) + \overline{b} -\underline{b} \le \theta \mathbbm{1}_n .
%%\end{align}
%\begin{align}
%& \left[  \begin{matrix}
% \underset{h(k)\in \mathbb{R}^{\xi}}  {\text{max}} & \left( \overline{G} -\underline{G} \right )h(k)   \\
%\text{s.t.}  & \hspace{-0.3cm} Q {h}(k)  \leq q
%\end{matrix} \right ] \le \theta \mathbbm{1}_n + \underline{b} - \overline{b} .
%\end{align}
%Taking the dual of the above inner maximization subproblem leads to 
%\begin{align}
%& \left[  \begin{matrix}
% \underset{\Pi \in \mathbb{R}^{k \times n} }  {\text{min}} & \hspace{-1.55cm} \Pi^\mathsf{T} q  \\
%\text{s.t.} &  \Pi^\mathsf{T} Q =  \overline{G} -\underline{G} \\
%& \hspace{-1.3cm} \Pi \ge 0
%\end{matrix} \right ] \le \theta \mathbbm{1}_n + \underline{b} - \overline{b} . \label{pAB_1:error}
%\end{align}
%
%With three inner minimization problems derived in \eqref{pAB_1:upper_ddual_final}, \eqref{pAB_1:lower_ddual_final} and \eqref{pAB_1:error}, we change the affine abstraction problem defined in Problem \ref{problem1} to a min-min problem. Moreover, dropping the inner minimization operators, the affine abstraction problem can be equivalently converted to its robust counterpart, which is the following single level minimization problem:
%\begin{subequations} \label{p13}
%\begin{align}
% \nonumber \min_{\substack{ \theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}, \Pi \\ \overline{p}_{i,2}, \underline{p}_{i,1}, \overline{\Pi}_i, \underline{\Pi}_i }} \; & \theta \hspace{5.6cm} \hfill (P_{DR})\\ %[-0.2em]
%\text{s.t.} \hspace{0.5cm} 
%& \overline{\Pi}_i^\mathsf{T} q \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \overline{p}_{i,2} +  \overline{b}_i \\ \overline{p}_{i,2}  \end{bmatrix}, ~  \forall i \in [n], \\ 
%& \overline{\Pi}_i^\mathsf{T} Q  = \begin{bmatrix} ({G_u})_i -  (\overline{G})_i  \\ - I_{\xi} \end{bmatrix} , ~  \forall i \in [n],  \\
%& \overline{\Pi}_i \ge 0 , ~  \forall i \in [n], \\
%& \overline{p}_{i,2} \ge 0,  \,\, \forall i \in [n],  \\
%& \underline{\Pi}_i^\mathsf{T} q \le \begin{bmatrix} \left( ({G_l})_i -  ({G_u})_i \right) \underline{p}_{i,1} - \underline{b}_i \\ \underline{p}_{i,1}  \end{bmatrix}, ~  \forall i \in [n], \\ 
%& \underline{\Pi}_i^\mathsf{T} Q  = \begin{bmatrix} (\underline{G})_i -  ({G}_l)_i  \\ - I_{\xi} \end{bmatrix} , ~  \forall i \in [n], \\
%&  \underline{\Pi}_i \ge 0 , ~  \forall i \in [n], \\
%& \underline{p}_{i,1} \ge 0,  \,\, \forall i \in [n], \\
%& \Pi^\mathsf{T} q \le \theta \mathbbm{1}_n + \underline{b} - \overline{b},   \label{sep:c1}\\
%&  \Pi^\mathsf{T} Q =  \overline{G} -\underline{G} ,  \label{sep:c3}\\
%&  \Pi \ge 0 .  \label{sep:c3}
%\end{align}
%\end{subequations}
%
%
%
%



\subsection{Equivalent LP via Robustification}

Based on the definition of an interval matrix, the uncertainty of each row of the system matrix $G$ can be equivalently written as a $\xi$-dimensional hyperrectangle that is defined as
%\begin{align}
% (G)_i^\mathsf{T} \in \mathcal{G}_i = \left \{ g \in \mathbb{R}^{\xi} : L g \le d_i \right \}, \forall i \in [n],
%\end{align}
\begin{align}
\mathcal{G}_i = [G_{l,i1}, G_{u,i1}] \times \ldots \times [G_{l, i \xi}, G_{u, i \xi}] , \,\, \forall i \in [n]. 
\end{align}
Thus, we have $(G)_i^\mathsf{T} \in \mathcal{G}_i$, where $(G)_i \in \mathbb{R}^{1 \times \xi}$ represents the $i$th row of the matrix $G$.
% the matrix $L\in \mathbb{R}^{2\xi \times \xi}$ and vector $d_i \in \mathbb{R}^{2\xi}$ are defined as
%\begin{align}
%L = \begin{bmatrix} I_{\xi} \\ -I_{\xi} \end{bmatrix}, \; d_i = \begin{bmatrix} (G_{u})_i^\mathsf{T}  \\   -(G_{l})_i^\mathsf{T} \end{bmatrix} .
%\end{align}
Consequently, the Problem \ref{problem1} with row-wise uncertainty can be rewritten as 
\begin{subequations} 
\begin{align}
\nonumber \underset{\theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}} {\text{min}}  \quad & \sum_{i=1}^{n}  \theta_i \\ %[-0.2em]
\text{s.t.}  \hspace{0.7cm}
& \hspace{-0.1cm} \begin{array}{l} \label{p11:a}
 (\overline{G})_i  {h}(k) + \overline{b}_i   \geq (G)_i {h}(k) ,  \\ \vspace{-0.05cm}
 \quad \forall (G)_i^\mathsf{T} \in \mathcal{G}_i, \forall h(k) \in \mathcal{H}, \forall i \in [n],   
\end{array} \\
& \hspace{-0.1cm} \begin{array}{l}  \label{p11:b}
(\underline{G})_i {h}(k)  + \underline{b}_i   \le (G)_i {h}(k) , \\ \vspace{-0.05cm}
 \quad \forall (G)_i^\mathsf{T} \in \mathcal{G}_i, \forall h(k) \in \mathcal{H}, \forall i \in [n], 
\end{array} \\
&  \hspace{-0.1cm}  \begin{array}{l} \label{p11:c} 
 \overline{f}_i \left( h(k) \right)- \underline{f}_i \left( h(k) \right)\le \theta_i , \\ \vspace{-0.05cm}
\quad \forall h(k) \in \mathcal{H}, \forall i \in [n], 
\end{array}\end{align}
\end{subequations}
where $\theta_i$ is the approximation error of the $i$th row.
Moreover, we derive the following useful lemma:
\begin{lemma}\label{lem:1}
Let the vertex set of the $\xi$-dimensional hyperrectangle $\mathcal{G}_i$ be denoted as $\mathcal{V}^g_i = \{v^g_{i,1},\ldots,v^g_{i, \varrho }\}$ with $\varrho = |\mathcal{V}^g_i| \le 2^{\xi}$, where $\varrho = 2^{\xi}$ holds when $G_i$ is unstructured, i.e., all elements of $G_i$ are independent. 
The constraints 
\begin{align} 
h^\mathsf{T}(k) (\overline{G})_i^\mathsf{T} + \overline{b}_i \ge h^\mathsf{T}(k) v^g_{i,j}, \, \, \forall  j \in [\varrho], \label{lem:inequality11}\\
h^\mathsf{T}(k) (\underline{G})_i^\mathsf{T} + \underline{b}_i \le h^\mathsf{T}(k) v^g_{i,j}, \, \, \forall  j \in [\varrho],\label{lem:inequality12}
\end{align}
are equivalent to $ (\overline{G})_i h(k)  + \overline{b}_i \ge (G)_i h(k) , \, \, \forall   \, (G)_i^\mathsf{T} \in \mathcal{G}_i$ and $ (\underline{G})_i h(k) + \underline{b}_i \le (G)_i h(k) , \, \, \forall   \, (G)_i^\mathsf{T} \in \mathcal{G}_i$.
%Suppose that 
%\begin{align} 
%h^\mathsf{T}(k) (\overline{G})_i^\mathsf{T} + \overline{b}_i \ge h^\mathsf{T}(k) v^g_{i,j}, \, \, \forall  j \in [\varrho], \label{lem:inequality11}\\
%h^\mathsf{T}(k) (\underline{G})_i^\mathsf{T} + \underline{b}_i \le h^\mathsf{T}(k) v^g_{i,j}, \, \, \forall  j \in [\varrho]. \label{lem:inequality12}
%\end{align}
%Then, we have $h^\mathsf{T}(k) (\overline{G})_i^\mathsf{T} + \overline{b}_i \ge h^\mathsf{T}(k) (G)_i^{T}, \, \, \forall   \, (G)_i^\mathsf{T} \in \mathcal{G}_i$, and $h^\mathsf{T}(k) (\underline{G})_i^\mathsf{T} + \underline{b}_i \le h^\mathsf{T}(k) (G)_i^{T}, \, \, \forall   \, (G)_i^\mathsf{T} \in \mathcal{G}_i$.
\end{lemma}
\begin{proof}
Since $\mathcal{G}_i$ is a $\xi$-dimensional hyperrectangle with vertex set $\mathcal{V}^g_i = \{v^g_{i,1},\ldots,v^g_{i, \varrho}\}$, any point in $(G)_i^\mathsf{T} \in \mathcal{G}_i$ can be represented as 
\begin{align} \label{property_polytope}
(G)_i^\mathsf{T} =\sum_{j=1}^{\varrho} \alpha_j v^g_{i,j},
\end{align}
where $\alpha_j \geq 0$ and $\sum_{j=1}^{\varrho} \alpha_j=1$. 
Multiplying both sides of \eqref{lem:inequality11} and \eqref{lem:inequality12} by the nonnegative constant $\alpha_j$, we have
\begin{gather} 
\alpha_j h^\mathsf{T}(k) (\overline{G})_i^\mathsf{T} + \alpha_j \overline{b}_i \ge \alpha_j h^\mathsf{T}(k) v^g_{i,j}, \, \, \forall  j \in [\varrho], \label{lem:inequality21} \\
\alpha_j h^\mathsf{T}(k) (\underline{G})_i^\mathsf{T} + \alpha_j \underline{b}_i \le \alpha_j h^\mathsf{T}(k) v^g_{i,j}, \, \, \forall  j \in [\varrho]. \label{lem:inequality22}
\end{gather}
Furthermore, adding all of the $\varrho$ inequalities in \eqref{lem:inequality21} and \eqref{lem:inequality22} respectively yields
\begin{align}
\sum_{j=1}^{\varrho} \alpha_j h^\mathsf{T}(k) (\overline{G})_i^\mathsf{T} + \sum_{j=1}^{\varrho} \alpha_j \overline{b}_i\ge  \sum_{j=1}^{\varrho} \alpha_j h^\mathsf{T}(k) v^g_{i,j}, \\
\sum_{j=1}^{\varrho} \alpha_j h^\mathsf{T}(k) (\underline{G})_i^\mathsf{T} + \sum_{j=1}^{\varrho} \alpha_j \underline{b}_i \le  \sum_{j=1}^{\varrho} \alpha_j h^\mathsf{T}(k) v^g_{i,j}. 
\end{align}
In light of $\sum_{j=1}^{\varrho} \alpha_j=1$ and \eqref{property_polytope}, the sufficiency can be obtained directly. 
Conversely, suppose we have $ (\overline{G})_i h(k)  + \overline{b}_i \ge (G)_i h(k) , \, \, \forall   \, (G)_i^\mathsf{T} \in \mathcal{G}_i$ and $ (\underline{G})_i h(k) + \underline{b}_i \le (G)_i h(k) , \, \, \forall   \, (G)_i^\mathsf{T} \in \mathcal{G}_i$.
As the uncertain set $\mathcal{G}_i$ contains every point including all its vertices, it is obvious that \eqref{lem:inequality11} and \eqref{lem:inequality12} hold. 
This completes the proof.
\end{proof}

\begin{theorem} 
The affine abstraction problem defined in Problem \ref{problem1} is equivalent to the following LP problem: 
\begin{subequations} \label{p_ab}
\begin{align}
 \nonumber \min_{\substack{ \theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}, \\ \overline{p}_{i,j}, \underline{p}_{i,j}, \Pi_i}} \; &  \sum_{i=1}^{n}  \theta_i \hspace{5.03cm} \hfill (P_{AB})\\ %[-0.2em]
\text{s.t.} \hspace{0.5cm} 
& \overline{p}_{i,j}^\mathsf{T} q \le \overline{b}_i,  \forall i \in [n], \forall  j \in [\varrho],    \\
& Q^\mathsf{T} \overline{p}_{i,j} = v^g_{i,j} - (\overline{G})_i^\mathsf{T},  \forall  i \in [n], \forall  j \in [\varrho],  \\
& \overline{p}_{i,j} \ge 0, \forall i \in [n], \forall  j \in [\varrho], \\
& \underline{p}_{i,j}^\mathsf{T} q \le -\underline{b}_i,  \forall i \in [n], \forall  j \in [\varrho],  \\
& Q^\mathsf{T} \underline{p}_{i,j} = (\underline{G})_i^\mathsf{T} - v^g_{i,j} ,  \forall  i \in [n], \forall   j \in [\varrho], \\
& \underline{p}_{i,j} \ge 0,  \forall i \in [n], \forall   j \in [\varrho],  \\
& \Pi_i^\mathsf{T} q \le \theta_i + \underline{b}_i - \overline{b}_i,   \label{sep:c1}\\
&  \Pi_i^\mathsf{T} Q =  \left(\overline{G}\right)_i - \left(\underline{G}\right)_i ,  \label{sep:c3}\\
&  \Pi_i \ge 0 ,  \label{sep:c3}
\end{align}
\end{subequations}
where $\overline{p}_{i,j}$, $\underline{p}_{i,j}$ and $\Pi$ are dual variables.
\end{theorem}

\begin{proof}
Lemma \ref{lem:1} implies that we can only consider all the vertices of the $\xi$-dimensional hyperrectangle $\mathcal{G}_i$ instead of every point in it. This simplifies the multiplication of two uncertain variables in constraints \eqref{p11:a} and \eqref{p11:b}, so that the nonlinear uncertainty in Problem \ref{problem1} reduces to a linear uncertainty. As a consequence, the Problem \ref{problem1} can be further cast as 
\begin{subequations} \label{p12}
\begin{align}
\nonumber \underset{\theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}}{\text{min}} \quad & \sum_{i=1}^{n} \theta_i\\ 
\text{s.t.} \hspace{0.7cm}
& \hspace{-0.1cm} \begin{array}{l} \label{p12:a} 
{h}^\mathsf{T}(k) (\overline{G})_i^\mathsf{T}  + \overline{b}_i   \geq {h}^\mathsf{T}(k) v^g_{i,j}  ,  \\ \vspace{-0.05cm}
\quad \forall h(k) \in \mathcal{H},  \forall i \in [n], \forall  j \in [\varrho], 
\end{array} \\
& \hspace{-0.1cm} \begin{array}{l} \label{p12:b}
 {h}^\mathsf{T}(k) (\underline{G})_i^\mathsf{T}  + \underline{b}_i   \le  {h}^\mathsf{T}(k) v^g_{i,j}  ,  \\ \vspace{-0.05cm}
\quad \forall h(k) \in \mathcal{H}, \forall i \in [n], \forall  j \in [\varrho],  
\end{array} \\
&  \hspace{-0.1cm}  \begin{array}{l} \label{p12:c} 
 \overline{f}_i \left( h(k) \right)- \underline{f}_i \left( h(k) \right)\le \theta_i , \\ \vspace{-0.05cm}
\quad \forall h(k) \in \mathcal{H}, \forall i \in [n], 
\end{array}\end{align}
\end{subequations}
where $v^g_{i,j}$, as defined in Lemma \ref{lem:1}, denotes the vertex of the $\xi$-dimensional hyperrectangle $\mathcal{G}_i$.

Now, the above equivalent abstraction problem is in a standard formulation of the robust optimization, we can use the method presented in \cite{ben2009robust, bertsimas2011theory} to convert the semi-infinite constraints into a tractable formulation.
Specifically, for the upper hyperplane constraint in \eqref{p12:a}, it can be equivalently written as
\begin{align}
\begin{array}{l}
\left[  \begin{matrix}
\underset{h(k) \in \mathbb{R}^{\xi}}  {\text{max}}  & h^\mathsf{T}(k) \left( v^g_{i,j} - (\overline{G})_i^\mathsf{T} \right)  \\
\text{s.t.}  & \hspace{-1.3cm} Q {h}(k)  \leq q
\end{matrix} \right ] \le \overline{b}_i, \\
~ \forall i \in [n], \forall  j \in [\varrho].
\end{array}
\end{align}
We proceed by applying LP duality to the inner maximization subproblem, turning it into an inner minimization problem. Thus, we have
\begin{align}
\begin{array}{l} \label{rc:a}
\left[  \begin{matrix}
\underset{\overline{p}_{i,j} \in \mathbb{R}^{k}}  {\text{min}}  & \hspace{-2.5cm} \overline{p}_{i,j}^\mathsf{T} q  \\
\text{s.t.} &  Q^\mathsf{T} \overline{p}_{i,j} = v^g_{i,j} - (\overline{G})_i^\mathsf{T} \\
& \hspace{-1.9cm} \overline{p}_{i,j} \ge 0
\end{matrix} \right ] \le \overline{b}_i, \\
~ \forall i \in [n], \forall  j \in [\varrho]. 
\end{array}
\end{align}
\indent
Similarly, the lower hyperplane constraints in \eqref{p12:b} can also be rewritten as
\begin{align}
\begin{array}{l}
\left[  \begin{matrix}
\underset{h(k) \in \mathbb{R}^{\xi}}  {\text{max}} & h^\mathsf{T}(k) \left(  (\underline{G})_i^\mathsf{T} - v^g_{i,j} \right)  \\
\text{s.t.}  & \hspace{-1.3cm} Q {h}(k)  \leq q
\end{matrix} \right ] \le -\underline{b}_i, \\
~ \forall i \in [n], \forall  j \in [\varrho].
\end{array}
\end{align}
Then, by using linear duality for its inner maximization subproblem, the constraint becomes
\begin{align}
\begin{array}{l} \label{rc:b}
\left[  \begin{matrix}
\underset{\underline{p}_{i,j}\in \mathbb{R}^{k}}  {\text{min}} & \hspace{-2.4cm} \underline{p}_{i,j}^\mathsf{T} q  \\
\text{s.t.} &  Q^\mathsf{T} \underline{p}_{i,j} =  (\underline{G})_i^\mathsf{T} - v^g_{i,j}\\
& \hspace{-1.9cm} \underline{p}_{i,j} \ge 0
\end{matrix} \right ] \le -\underline{b}_i, \\
~ \forall i \in [n], \forall  j \in [\varrho]. 
\end{array}
\end{align}
\indent
Finally, for the constraint describing the upper bound of the approximation error in \eqref{p12:c}, we have
%due to the fact that
%\begin{align*}
% \|\overline{f} \left( h(k) \right) - \underline{f} \left( h(k) \right) \|_\infty = \max_{i \in [n]} \;( \overline{f}_i \left( h(k) \right)- \underline{f}_i \left( h(k) \right) ), 
% \end{align*}
%it can be written as
%\begin{align}
% \max_{h(k) \in \mathcal{H}} \max_{i \in [n]} \; ( \overline{f}_i \left( h(k) \right)- \underline{f}_i \left( h(k) \right) ) \le \theta ,
% \end{align}
% which further implies that 
%% \begin{align}
%% \max_{h(k) \in \mathcal{H}}  \; \overline{G} h(k) -\underline{G} h(k) + \overline{b} -\underline{b} \le \theta \mathbbm{1}_n .
%%\end{align}
\begin{align}
\begin{array}{l} \label{rc:b}
 \left[  \begin{matrix}
 \underset{h(k)\in \mathbb{R}^{\xi}}  {\text{max}} & \left( \left(\overline{G}\right)_i - \left(\underline{G}\right)_i \right )h(k)   \\
\text{s.t.}  & \hspace{-1.2cm} Q {h}(k)  \leq q
\end{matrix} \right ] \le \theta_i + \underline{b}_i - \overline{b}_i ,  \\
 ~ \forall i \in [n]. 
\end{array}
\end{align}
Taking the dual of the above inner maximization leads to 
\begin{align}
\begin{array}{l} \label{rc:c}
\left[  \begin{matrix}
 \underset{\Pi_i \in \mathbb{R}^{k} }  {\text{min}} & \hspace{-2.4cm} \Pi_i^\mathsf{T} q  \\
\text{s.t.} &  \Pi_i^\mathsf{T} Q =  \left(\overline{G} \right)_i- \left(\underline{G} \right)_i\\
& \hspace{-2cm}  \Pi_i \ge 0
\end{matrix} \right ] \le \theta_i + \underline{b}_i - \overline{b}_i ,  \\
~  \forall i \in [n].
\end{array}
\end{align}

With these three inner minimization subproblems derived in \eqref{rc:a}, \eqref{rc:b} and \eqref{rc:c}, we can convert the affine abstraction problem defined in Problem \ref{problem1} into a tractable problem. 
Note that dropping the inner minimization operator and regarding the decision variables of the inner minimization as additional variables to the outer minimization would not change the optimal value \cite{bertsimas2011theory, ben2009robust}. 
Thus, the affine abstraction problem can be equivalently recast to its robust counterpart (RC), which is the single level LP problem ($P_{AB}$). 
\end{proof}
%\begin{subequations} \label{p_ab}
%\begin{align}
% \nonumber \min_{\substack{ \theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}, \\ \overline{p}_{i,j}, \underline{p}_{i,j}, \Pi}} \; & \theta \hspace{5.95cm} \hfill (P_{AB})\\ %[-0.2em]
%\text{s.t.} \hspace{0.5cm} 
%& \overline{p}_{i,j}^\mathsf{T} q \le \overline{b}_i,  \forall i \in [n], \forall  j \in [\varrho],    \\
%& Q^\mathsf{T} \overline{p}_{i,j} = v^g_{i,j} - (\overline{G})_i^\mathsf{T},  \forall  i \in [n], \forall  j \in [\varrho],  \\
%& \overline{p}_{i,j} \ge 0, \forall i \in [n], \forall  j \in [\varrho], \\
%& \underline{p}_{i,j}^\mathsf{T} q \le -\underline{b}_i,  \forall i \in [n], \forall  j \in [\varrho],  \\
%& Q^\mathsf{T} \underline{p}_{i,j} = (\underline{G})_i^\mathsf{T} - v^g_{i,j} ,  \forall  i \in [n], \forall   j \in [\varrho], \\
%& \underline{p}_{i,j} \ge 0,  \forall i \in [n], \forall   j \in [\varrho],  \\
%& \Pi^\mathsf{T} q \le \theta \mathbbm{1}_n + \underline{b} - \overline{b},   \label{sep:c1}\\
%&  \Pi^\mathsf{T} Q =  \overline{G} -\underline{G} ,  \label{sep:c3}\\
%&  \Pi \ge 0 .  \label{sep:c3}
%\end{align}
%\end{subequations}

Since ($P_{AB}$) is an LP, it can be solved efficiently. 
As for the computational complexity of the proposed approach ($P_{AB}$), it is observed that there are $1+2n+kn+2n\xi+kn\varrho$ decision variables with $n(\xi+1)(2 \varrho +1)$ linear constraints. 
However, the number of vertices (e.g., $\varrho$) increases exponentially with respect to the increase of  system dimension.


\begin{proposition} \label{propos1}
If the system state $x(k)$, control input $u(k)$, process noise $w(k)$ and the unknown constant vector $f$ are also constrained by closed interval domains $\mathcal{X} = [a_{x,1}, b_{x,1}] \times \ldots \times [a_{x,n}, b_{x,n}] \subset \mathbb{R}^n$, $\mathcal{U} = [a_{u,1}, b_{u,1}] \times \ldots  \times [a_{u,m}, b_{u,m}] \subset \mathbb{R}^m$, $\mathcal{W}  = [a_{w,1}, b_{w,1}] \times \ldots \times [a_{w,m_w}, b_{w,m_w}]  \subset \mathbb{R}^{m_w}$ and $\mathcal{F} = [a_{f,1}, b_{f,1}] \times \ldots \times [a_{f,m_f}, b_{f,m_f}]  \subset \mathbb{R}^{m_f}$, then the constraints \eqref{sep:c1}-\eqref{sep:c3} in the affine abstraction problem ($P_{AB}$) can be replaced by 
\begin{align}
\left( \left(\overline{G}\right)_i -\left(\underline{G} \right )_i \right) v^h_{j} + \overline{b}_i - \underline{b}_i \le \theta_i, \,\,  \forall i \in [n], \forall   j \in [2^{\xi}],  \label{propos_constr}
\end{align}
where $v^h_{j} \in \mathcal{V}^h = \{v^h_{1}, \ldots, v^h_{2^{\xi} }\}$ is the vertex set of the $\xi$-dimensional hyperrectangle $\mathcal{H}_p$ defined in the proof.
\end{proposition}

\begin{proof}
Based on the definition of interval matrices, the augmented state $h (k) = \begin{bmatrix} x(k)& u(k)& w(k)& f \end{bmatrix}^\mathsf{T} \in \mathbb{R}^{\xi}$ is aslo constrained by a $\xi$-dimensional hyperrectangle defined as $\mathcal{H}_p= \mathcal{X} \times \mathcal{U} \times \mathcal{W} \times \mathcal{F}$,
which can be equivalently written as polyhedral set $\mathcal{H}_p = \left \{  h \in \mathbb{R}^{\xi} : Q h \le q \right \}$, where 
\begin{align}
Q = & \begin{bmatrix} I_{\xi} & -I_{\xi} \end{bmatrix} ^\mathsf{T} \in \mathbb{R}^{2 \xi \times \xi} , \notag \\
q = & \begin{bmatrix} b^\mathsf{T}_x  \;\;\;  b^\mathsf{T}_u \;\;\;  b^\mathsf{T}_w \;\;\; b^\mathsf{T}_f \;\, -a^\mathsf{T}_x \;\,  -a^\mathsf{T}_u \;\, -a^\mathsf{T}_w \;\, -a^\mathsf{T}_f  \end{bmatrix}^\mathsf{T} \in \mathbb{R}^{2\xi}.\notag
\end{align}
In this case, for the constraint \eqref{p12:c}, consider any one dimension in $\mathbb{R}^{\xi}$ with the other dimensions arbitrarily fixed. Due to the linear nature of the difference between $\overline{f}$ and $\underline{f}$, the difference can only be increasing or decreasing as the augmented state moves in one direction. Due to this observation, the maximum difference would be at one of the ends. Since this argument applies to all dimensions, it follows that the maximum difference must be attained at one of the vertices of $\mathcal{H}_p$. 
In view of this, we do not have to apply robust optimization to the constraint of the approximation error and only need to minimize the difference among the vertices of the $\xi$-dimensional hyperrectangle. 
Therefore, the constraint \eqref{p12:c} can be equivalently replaced by \eqref{propos_constr}. 
\end{proof}

As a result of the additional assumption in Proposition \ref{propos1}, the abstraction problem ($P_{AB}$) has $1+2n+2n\xi+nk\varrho$ decision variables and $n(2^{\xi}+2\varrho+2\xi \varrho)$ linear constraints, which indicates that we have $kn$ less decision variables but $n(2^\xi-\xi-1)$ more linear constraints when compared to the optimization formulation in \eqref{p_ab}. Note that since $\xi$ is the total number of states, control inputs, noise, and additive faults, $\xi \ge 1$ always holds and $n(2^\xi-\xi-1) \geq 0$.


\begin{remark}
In most affine systems, the noise matrix $B_w$ and the fault matrix $B_f$ are fixed. Thus, the compact form of the uncertain affine system \eqref{dynamics} can be written  as
\begin{align*}
x(k+1) = G_1 h_1(k) + G_2 h_2(k), 
\end{align*}
where the augmented uncertain system matrix $G_1 = \begin{bmatrix} A  & B \end{bmatrix} \in G_1^{I} \subset \mathbb{R}^{n \times {\xi_1}}$ and the fixed matrix $G_2 = \begin{bmatrix} B_w & B_f \end{bmatrix} \in  \mathbb{R}^{n \times {\xi_2}}$ with $\xi_1 = n+m$ and $\xi_2 = m_w +m_f$, and the corresponding augmented states $h_1 (k) = \begin{bmatrix} x^\mathsf{T}(k)& u^\mathsf{T}(k)\end{bmatrix}^\mathsf{T} \in \mathcal{H}_1 \subset \mathbb{R}^{\xi_1}$ and $h_2 (k) = \begin{bmatrix} w^\mathsf{T}(k)& f ^\mathsf{T}\end{bmatrix}^\mathsf{T} \in \mathcal{H}_2 \subset \mathbb{R}^{\xi_2}$.
Then, the lower and upper hyperplanes for the abstraction are defined as
\begin{align*}
\underline{f} = \underline{G}_1 h_1(k) + \underline{b}_1 + G_2 h_2(k), \\
\overline{f} = \overline{G}_1 h_1(k) + \overline{b}_1 + G_2 h_2(k).
\end{align*}
Then, the affine abstraction is formulated as
\begin{subequations}
\begin{align*} 
 \nonumber \min_{\substack{ \overline{G}_1, \underline{G}_1, \overline{b}_1, \underline{b}_1,  \theta}} \quad &\theta   \\  
\text{s.t.} \hspace{1cm} 
& \hspace{-0.1cm}  \begin{array}{l}   
\overline{G_1} \, {h}(k) + \overline{b}_1  \geq G_1 {h}(k) ,  \\
\quad \forall \,G_1 \in G_1^I, \forall \, h_1(k) \in \mathcal{H}_1,  
\end{array} \\ 
& \hspace{-0.1cm}   \begin{array}{l} 
\underline{G}_1 \, {h}(k) + \underline{b}_1  \leq G_1 {h}(k), \\
\quad \forall \,G_1 \in G_1^I, \forall \, h_1(k) \in \mathcal{H}_1, 
\end{array} \\
&   \max_{h_1(k) \in \mathcal{H}_1} \| \overline{f} - \underline{f} \|_1 \le \theta .
\end{align*}
\end{subequations}
Since we only consider the uncertainties on $G_1$ and $h_1(k)$, the above formulation has a lower dimension and complexity.
Following the same procedures in solving the Problem \ref{problem1}, we can also obtain the solution of the above low-dimensional affine abstraction problem (omitted for brevity).
\end{remark}


%\begin{table}[ht] %\vspace{-0.3cm}
%	\centering
%	\caption{Complexity of the double robustification and single robustification formulations.} %\vspace{0.1cm}
%	\label{table:numerical2}
%	\begin{tabular}{c c c}
%		\hline
%	Formulation & No. of constraints & No. of variables\\ 
%		\hline
%	\begin{tabular}{@{}c@{}}Double \\ Robustification \end{tabular} & $n(\xi+1)(2\xi+3)$ & $1+2n+8n\xi+4kn\xi$ \\[1ex]
%		\hline
%	\begin{tabular}{@{}c@{}}Single \\ Robustification \end{tabular} & $n(\xi+1)(2^{\xi+1}+1)$ & \begin{tabular}{@{}c@{}}$1+2n+kn$ \\ $+2n\xi+kn\varrho$ \end{tabular} \\[1ex]
%		\hline
%	\end{tabular}
%\end{table}





%  \newpage

%The original system:
%\begin{align*}
%x(k+1) = A \, x(k), \, A \in [A_{l},A_{u}]
%\end{align*}
%Here, $A, \, A_{l}$ and $A_{u}$ are $n \times n$ dimensional matrix. The lower and upper bound of each element in $A$ is the respective element in $A_{l}$ and $A_{u}$ respectively. We want to find $\overline{A}$ and $\underline{A}$ such that:
%\begin{align} \label{both}
%\begin{split}
%&\underline{A} \, x(k) \leq A \, x(k) \leq \overline{A} \, x(k), \\
% &\forall A \in  [A_{l},A_{u}], \forall x \in \{x:Q \, x \leq q\}
%\end{split}
%\end{align}
%Here $Q$ and $q$ are used to define the polyhedral domain of $x$. We break these two inequalities into individual uncertain constraints and then use robust optimization to make them solvable:
%\begin{align}
%\begin{split}
%A \, x(k) \leq \overline{A} \, x(k), \, \forall A \in  [A_{l},A_{u}],\\
%\forall x \in \{x:Q \, x \leq q\}
%\end{split}
%\end{align}
%
%\begin{subequations} \label{uncertain}
%\begin{equation} \label{uncertain_a}
%\implies (\max A\,x(k)) \leq \overline{A} \, x(k)
%\end{equation}    
%\begin{equation} \label{uncertain_b}
%s.t. \,\, G \, vec(A) \leq d
%\end{equation}
%\end{subequations} 
%where:
%\begin{align*}
%vec(A) = 
%\begin{bmatrix} 
%a_{1} & a_{2} & \hdots & a_{n}
%\end{bmatrix}^{T}
%\end{align*}
%$a_{1}$ through $a_{m}$ are respective rows of $A$
%\begin{align*}
%G = 
%%\begin{bmatrix} 
%%I & 0 & \hdots & 0\\
%%0 & I & \hdots & 0\\
%%\vdots & \vdots & \cdots & \vdots\\
%%0 & 0 & \hdots & I\\
%%-I & 0 & \hdots & 0\\
%%0 & -I & \hdots & 0\\
%%\vdots & \vdots & \cdots & \vdots\\
%%0 & 0 & \hdots & -I
%%\end{bmatrix}_{2 \, m \times m}
%\begin{bmatrix} 
%I\\
%-I
%\end{bmatrix} \in \mathbb{R}^{2n^2 \times n^2}
%\end{align*}
%
%\begin{align*}
%d = 
%\begin{bmatrix} 
%vec(A_{u}) \\
%vec(A_{l})
%\end{bmatrix} \in \mathbb{R}^{2n^2}
%\end{align*}
%Using duality with (\ref{uncertain}):
%
%\begin{subequations} \label{dual}
%\begin{equation} \label{dual_a}
%\begin{split}
%\implies (\min p_{u,i}^{T}\,d) \leq \overline{A}_{(i,:)} \, x& \\
%\forall x \in \mathcal{X}, \, \, \forall i \in \{1,2,\hdots,n\}& 
%\end{split}
%\end{equation}    
%\begin{equation} \label{dual_b}
%s.t. \,\, G^{T} \, p_{u,i} = x_{i} \, \, \, \forall x \in \mathcal{X}
%\end{equation}
%\begin{equation} \label{dual_c}
%p_{u,i}^{T} \geq 0
%\end{equation}
%\end{subequations}
%
%\begin{equation*}
%x_{i} = 
%\begin{bmatrix}
%(0_{n \times 1})_{1}\\
%(0_{n \times 1})_{2}\\
%\vdots \\
%(x_{n \times 1})_{i}\\
%\vdots \\
%(0_{n \times 1})_{n}
%\end{bmatrix} \in \mathbb{R}^{n^2}
%\end{equation*}
%
%Here, $x$ is at the $i^{th}$ position in $x_{i}$. From (\ref{dual_b}), we get three set of equations:
%
%\begin{subequations} \label{ext}
%\begin{equation} \label{ext_a}
%x = G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{u,i}
%\end{equation}
%\begin{equation} \label{ext_b}
%G^{T}([1 \, \, \, n(i-1)],:) \, p_{u,i} = 0
%\end{equation}
%\begin{equation} \label{ext_c}
%G^{T}([n\, i+1 \, \, \, n^{2}],:) \, p_{u,i} = 0
%\end{equation}
%\end{subequations}
%
%(\ref{ext_b}) doesn't apply for $i = 1$ and (\ref{ext_c}) doesn't apply for  $i = n$. \\
%Applying (\ref{ext_a}) to (\ref{dual_a}) and disregarding the $\min$:
%
%\begin{subequations}
%\begin{equation}
%\begin{split}
%p_{u,i}^{T}\,d \leq \overline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{u,i}\\
%\forall i \in \{1,2, \hdots, n\}
%\end{split}
%\end{equation}
%\begin{equation}
%\begin{split}
%Q \,  G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{u,i} \leq q \\
%\forall i \in \{1,2, \hdots, n\}
%\end{split}
%\end{equation}
%\end{subequations}
%
%Since $p_{u,i}^{T}\,d$ results in a scalar, we can substitute it with $d^{T} \, p_{u,i}$:
%\begin{align*}
%\begin{split}
%\implies  d^{T}\,p_{u,i} \leq \overline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{u,i},&\\
% \forall i \in \{1,2, \hdots ,n\}&
%\end{split}
%\end{align*}
%
%\begin{align}
%\begin{split}
%\implies (d^{T} -  \overline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:)) \, p_{u,i} \leq 0,&\\
% \forall i \in \{1,2, \hdots ,n\} &
%\end{split}
%\end{align}
%
%So instead of (\ref{uncertain}) we have $n$ optimization problems of the following form:
%
%\begin{align*}
%\max \, &(d^{T} -  \overline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:)) \, p_{u,i} \leq 0 \\
%s.t. \,\,\, & Q \,  G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{u,i} \leq q \\
%&G^{T}([1 \, \, \, n(i-1)],:) \, p_{u,i} = 0 \\
%&G^{T}([n\, i+1 \, \, \, n^{2}],:) \, p_{u,i} = 0\\
%&p_{u,i} \geq 0
%\end{align*}
%
%Using shorthand matrices for the above problem:
%
%\begin{align} \label{robust1}
%\begin{split}
%\implies \,\, \max \,\,\, &\overline{\Omega}_{i} \, p_{u,i} \leq 0 \\
%s.t. \,\,\, & \overline{\Theta}_{i} \, p_{u,i} \leq q \\
%& \overline{\Gamma}_{i} \, p_{u,i} = 0 \\
%&p_{u,i} \geq 0
%\end{split}
%\end{align}
%
%Here, $\overline{\Theta}_{i}$ and $\overline{\Gamma}_{i}$ are independent of any decision variables. But $\overline{\Omega}_{i}$ includes decision variables ($\overline{A}$ elements). Since $\overline{\Omega}_{i}$ multiplies with $p_{u,i}$, we need to further robustify this problem. Applying duality to (\ref{robust1}).
%
%\begin{align}\label{robust2}
%\begin{split}
%\min \,\,\, & q^{T} \, y_{1}^{i} \leq 0\\
%& \overline{\Theta}_{i}^{T} \, y_{1}^{i} + \overline{\Gamma}_{i}^{T} \, y_{2}^{i}  \geq \overline{\Omega}_{i}\\
%& y_{1}^{i} \geq 0\\
%& y_{2}^{i} \geq 0
%\end{split}
%\end{align}
%
%disregarding the $\min$ again, we have the above four constraints instead of (\ref{uncertain}) and decision variables are $y_{1}^{i}$, $y_{2}^{i}$ and elements of $\overline{A}$. As we can see in (\ref{robust2}), all of these decision variables are independent, making the bigger problem now solvable with these constraints. 
%\\ \\
%Similarly for the other inequality in (\ref{both}):\\
%
%\begin{align*}
%\begin{split}
%\underline{A} \, x(k) \leq A \, x(k), \, \forall A \in  [A_{l},A_{u}],\\
%\forall x \in \{x:Q \, x \leq q\}
%\end{split}
%\end{align*}
%\begin{align}
%\begin{split}
%\implies -A \, x(k)  \leq -\underline{A} \, x(k), \, \forall A \in  [A_{l},A_{u}],\\
%\forall x \in \{x:Q \, x \leq q\}
%\end{split}
%\end{align}
%
%
%\begin{subequations} \label{uncertain2}
%\begin{equation} \label{uncertain2_a}
%\implies \max (-A\,x(k)) \leq -\underline{A} \, x(k)
%\end{equation}    
%\begin{equation} \label{uncertain2_b}
%s.t. \,\, G \, vec(A) \leq d
%\end{equation}
%\end{subequations} 
%
%
%\begin{subequations} \label{dual2}
%\begin{equation} \label{dual2_a}
%\implies (\min p_{l,i}^{T}\,d) \leq -\underline{A}_{(i,:)} \, x \, \, \, \forall x \in \mathcal{X}
%\end{equation}    
%\begin{equation} \label{dual2_b}
%s.t. \,\, p_{l,i}^{T} \, G = x^{T} \, \, \, \forall x \in \mathcal{X}
%\end{equation}
%\begin{equation} \label{dual2_c}
%p_{l,i}^{T} \geq 0
%\end{equation}
%\end{subequations}
%
%From (\ref{dual2_b}), we get three set of equations:
%
%\begin{subequations} \label{ext2}
%\begin{equation} \label{ext2_a}
%x = G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{l,i}
%\end{equation}
%\begin{equation} \label{ext2_b}
%G^{T}([1 \, \, \, n(i-1)],:) \, p_{l,i} = 0
%\end{equation}
%\begin{equation} \label{ext2_c}
%G^{T}([n\, i+1 \, \, \, n^{2}],:) \, p_{l,i} = 0
%\end{equation}
%\end{subequations}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%(\ref{ext2_b}) doesn't apply for $i = 1$ and (\ref{ext2_c}) doesn't apply for  $i = n$. \\
%Applying (\ref{ext2_a}) to (\ref{dual2_a}) and disregarding the $\min$:
%
%\begin{subequations}
%\begin{equation}
%\begin{split}
%p_{l,i}^{T}\,d \leq -\underline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{u,i}\\
%\forall i \in \{1,2, \hdots, n\}
%\end{split}
%\end{equation}
%\begin{equation}
%\begin{split}
%Q \,  G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{l,i} \leq q \\
%\forall i \in \{1,2, \hdots, n\}
%\end{split}
%\end{equation}
%\end{subequations}
%
%Since $p_{l,i}^{T}\,d$ results in a scalar, we can substitute it with $d^{T} \, p_{l,i}$:
%\begin{align*}
%\begin{split}
%\implies  d^{T}\,p_{l,i} \leq -\underline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{l,i},&\\
% \forall i \in \{1,2, \hdots ,n\}&
%\end{split}
%\end{align*}
%
%\begin{align}
%\begin{split}
%\implies (d^{T} +  \underline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:)) \, p_{l,i} \leq 0,&\\
% \forall i \in \{1,2, \hdots ,n\} &
%\end{split}
%\end{align}
%
%So instead of (\ref{uncertain2}) we have $n$ optimization problems of the following form:
%
%\begin{align*}
%\max \, &(d^{T} +  \underline{A}_{(i,:)} \,   G^{T}([n(i-1)+1 \, \, \, n \, i],:)) \, p_{l,i} \leq 0 \\
%s.t. \,\,\, & Q \,  G^{T}([n(i-1)+1 \, \, \, n \, i],:) \, p_{l,i} \leq q \\
%&G^{T}([1 \, \, \, n(i-1)],:) \, p_{l,i} = 0 \\
%&G^{T}([n\, i+1 \, \, \, n^{2}],:) \, p_{l,i} = 0\\
%&p_{l,i} \geq 0
%\end{align*}
%
%Using shorthand matrices for the above problem:
%
%\begin{align} \label{robust1_l}
%\begin{split}
%\implies \,\, \max \,\,\, &\underline{\Omega}_{i} \, p_{l,i} \leq 0 \\
%s.t. \,\,\, & \underline{\Theta}_{i} \, p_{l,i} \leq q \\
%& \underline{\Gamma}_{i} \, p_{l,i} = 0 \\
%&p_{l,i} \geq 0
%\end{split}
%\end{align}
%
%Here, $\underline{\Theta}_{i}$ and $\underline{\Gamma}_{i}$ are independent of any decision variables. But $\underline{\Omega}_{i}$ includes decision variables ($\underline{A}$ elements). Since $\underline{\Omega}_{i}$ multiplies with $p_{l,i}$, we need to further robustify this problem. Applying duality to (\ref{robust1_l}).
%
%\begin{align}\label{robust2_l}
%\begin{split}
%\min \,\,\, & q^{T} \, z_{1}^{i} \leq 0\\
%& \underline{\Theta}_{i}^{T} \, z_{1}^{i} + \underline{\Gamma}_{i}^{T} \, z_{2}^{i}  \geq \underline{\Omega}_{i}\\
%& z_{1}^{i} \geq 0\\
%& z_{2}^{i} \geq 0
%\end{split}
%\end{align}
%
%So we finally have the same optimization problem as in CDC with added constraints (\ref{robust2}) and (\ref{robust2_l}):














%Given a nonlinear function $f: I\rightarrow \mathbb{R}^n$ with a hyperrectangular domain $I \subset \mathbb{R}^{n+m}$ for any subregion $I \in \mathcal{I}$, 

%let $\mathcal{V} = \{{v}_{1}, {v}_{2}, \hdots, {v}_{l} \}$ be a set of $l$ grid points of a uniform mesh of $\mathcal{X}$. $\mathcal{C} =  \{ {v}^{c}_{1}, \ldots, {v}^{c}_{2^{(n+m)}} \}$ be a set of the corner points of $\mathcal{X}$.
%The affine hyperplanes $\overline{f}$ and $\underline{f}$ that over-approximate/abstract $f$ are given by:
%\begin{align*}
%\overline{f} = f_{u} + \sigma, \quad 
%\underline{f} = f_{b} - \sigma,
%\end{align*}
%Since the system here is affine, $\sigma$ would be $0$.
%%\begin{align*}
%$f_{u} = \overline{A}\,x,$ and %\quad 
%$f_{b} = \underline{A}\,x$, 
%%\end{align*}
%where $\overline{A}$ and $\underline{A}$ are obtained from the following linear programming (LP) problem:
%%\begin{equation*} %\label{min_prob}
%\begin{subequations} 
%\begin{align}
%\nonumber &\underset{\theta, \overline{A}, \underline{A}, \overline{B}, \underline{B}, h_{u},h_{b}}{\text{min}}
% \theta \\[-0.2em]
%&\text{subject to} \quad 
%\overline{A}\, {x}_{i} \geq f({x}_{i}), \label{eq:a}\\[-0.2em]
%& \hspace{1.75cm} \underline{A}\, {x}_{i} \leq f({x}_{i}), \label{eq:b}\\[-0.2em]
%& \hspace{0.7cm} (\overline{A} - \underline{A}) \, {x}^{c}_{j} \leq \theta, \label{eq:c} \\[-0.2em]
%\nonumber & \hspace{1.75cm} \forall i \in [l], \forall j\in [2^{(n+m)}], 
%\end{align}
%\end{subequations}
%where $(x_i)$ and $(x^c_j)$ are the state-input values at the grid point $v_i$ of the mesh and the vertex $c_j$, respectively.



























%in \ref{dual_a}, we can disregard the min and use this inquality as a constraint (still to be robustified since $x$ is in a range).

%\begin{align}
%p_{u,i}^{T}\,d \leq \overline{A}_{(i,:)} \, x \, \, \, \forall x \in \mathcal{X}   \, \, \forall i \in \mathcal{Z}_{m}^{+}
%\end{align}




%

%
%\begin{align}
%p_{l,i}^{T}\,d \leq \underline{A}_{(i,:)} \, x \, \, \, \forall x \in \mathcal{X}   \, \, \forall i 
%\end{align}
%
%As of now we have variable matrices $\underline{A}$, $\overline{A}$, variable vectors $p_{l}$, $p_{u}$ due to robustification of the two origianl constraints ((\ref{uncertain}) and (\ref{uncertain2})) and still the uncertain variable vector $x$. Now robutifying w.r.t. $x$:


==> sec_examples.tex <==
%!TEX root = main.tex
\section{Simulation Examples}
In this section, we apply the proposed affine abstraction to over-approximate uncertain intention models of other human-driven vehicles in the scenario of the intersection crossing.

\subsection{Vehicle and Intention Models}
Consider two vehicles at an intersection, which is the origin of the coordinate system.
The discrete-time equations governing the motion of two vehicles are given in \cite{Ding2018}:
\begin{align*}
x_{e}(k+1) &= x_{e}(k) + v_{x,e}(k) \delta t, \\
v_{x,e}(k+1) &= v_{x,e}(k) + u(k) \delta t + w_{x}(k) \delta t, \\
y_{o}(k+1) &= y_{o}(k) + v_{y,o}(k) \delta t,\\
v_{y,o}(k+1) &= v_{y,o}(k) + d_{i}(k) \delta t + w_{y}(k) \delta t,
\end{align*}
where $x_e$ and $v_{x,e}$ are ego car's position and velocity, $y_{o}$ and $v_{y,o}$ are other car's position and velocity, $w_x$ and $w_y$ are process noise, and $\delta t = 0.3$ s is the sampling time. $u$ is the acceleration input for ego car, whereas $d_i$ is the acceleration input of the other car for each intention $i \in \{C, M, I\}$, corresponding to \underline{C}autious, \underline{M}alicious or \underline{I}nattentive driver. 

As illustrated in \cite{Ding2018}, we use a PD controller to model driver's intention. However, the control gains in these intention models cannot be exactly obtained due to the complexity of the human's driving behavior. 
The \textbf{Cautious} driver drives carefully and tends to stop at the intersection with an input equal to $d_C \triangleq -K_{p,C} y_o(k) -K_{d,C} v_{y,o}(k) + \tilde{d}_C(k)$, where the uncertain PD controller parameters $K_{p,C} \in [0, 1.8]$ and $K_{d,C} \in [0, 5.5]$ represent characteristics of the cautious driver, and $\tilde{d}_C(k) \in \mathcal{D}_C = [-0.392, 0.198]$ m/$\text{s}^\text{2}$ denotes the unmodeled variations accounting for nondeterministic driving behaviors.
The \textbf{Malicious} driver drives aggressively and attempts to cause a collision with an input $d_M \triangleq K_{p,M} (x_e(k) - y_o(k)) + K_{d,M} (v_{x,e}(k) - v_{y,o}(k) )+ \tilde{d}_M(k)$, where $K_{p,M} \in [0, 2]$ and $K_{d,M} \in [0, 5]$ are PD controller parameters, % that represent characteristics of the malicious driver
and $\tilde{d}_M(k) \in \mathcal{D}_M = [-0.392, 0.198]$ m/$\text{s}^\text{2}$.
Finally, the \textbf{Inattentive} driver is unaware of the ego car and attempts to maintain its speed with an uncontrolled acceleration input $d_I(k)  \in \mathcal{D}_C = [-0.784, 0.396]$ m/$\text{s}^\text{2}$. 

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\vspace{-0.1cm}
\centering
\includegraphics[width = 2.4in]{C_result.eps}
\caption{Affine abstraction of the uncertain dynamics of \textbf{cautious} driver's velocity in $(y_o, v_{y,o})$ plane of projection when $w_y(k) = 0$ and $\tilde{d}_C(k) = 0$. The red and the blue hyperplanes are upper and lower hyperplanes obtained from abstraction, while the uncertain set is the meshed region.} 
\label{fig:C_result}
\end{figure}
%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\vspace{-0.05cm}
\centering
\subfloat[$(x_e, v_{x,e})$ projection plane]{\includegraphics[width=1.7in]{M_result1.eps}%
\label{M_result1}}
\hfil
\subfloat[$(x_e, y_{o})$ projection plane]{\includegraphics[width=1.7in]{M_result2.eps}%
\label{M_result2}}
\vspace{-0.05in}
\hfil
\subfloat[$(x_e, v_{y,o})$ projection plane]{\includegraphics[width=1.7in]{M_result3.eps}%
\label{M_result3}}
\hfil
\subfloat[$(v_{x,e}, y_{o})$ projection plane]{\includegraphics[width=1.7in]{M_result4.eps}%
\label{M_result4}}
\vspace{-0.05in}
\hfil
\subfloat[$(v_{x,e}, v_{y,o})$ projection plane]{\includegraphics[width=1.7in]{M_result5.eps}%
\label{M_result5}}
\hfil
\subfloat[$(y_{o}, v_{y,o})$ projection plane]{\includegraphics[width=1.7in]{M_result6.eps}%
\label{M_result6}}
\caption{Affine abstraction of the uncertain dynamics of \textbf{malicious} driver's velocity in different projection planes when $w_y(k) = 0$ and $\tilde{d}_M(k) = 0$.}
\label{fig:M_result}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Substituting intention models to the dynamics of the other vehicle, the equation governing the other car's velocity under different intentions becomes: \\
\noindent\textbf{Cautious Driver} $(i=\text{C})$: 
\begin{align} \label{C_intention}
v_{y,o}(k+1) = & - \delta t K_{p,C} y_o(k) + (1- \delta t K_{d,C} ) v_{y,o}(k)  \notag \\
& + \delta t w_{y}(k) + \delta t \tilde{d}_C(k),
\end{align}
\textbf{Malicious Driver} $(i=\text{M})$: 
\begin{align} \label{M_intention}
v_{y,o}(k+1) = &  \delta t K_{p,M} x_e(k) + \delta t K_{d,M} v_{x,e}(k)  \notag \\
& - \delta t K_{p,M} y_o(k) + (1- \delta t K_{d,M} ) v_{y,o}(k)   \notag \\
& + \delta t w_{y}(k) + \delta t \tilde{d}_M(k),
\end{align}
\textbf{Inattentive Driver} $(i=\text{I})$: 
\begin{align} \label{I_intention}
v_{y,o}(k+1) = v_{y,o}(k)  + \delta t w_{y}(k) + \delta t {d}_I(k).
\end{align}

Moreover, we assume that the ego car's position is constrained to be between $[0,18]$ m at all times, and its velocity is between $[0,9]$ m/s. The other car's position is between $[-18,18]$ m, while its velocity is between $[-9,9]$ m/s. The process noise signals are bounded to $[-0.01, 0.01]$.

\subsection{Affine Abstraction}

Since the uncertain PD parameters only affect the other car's velocity $v_{y,o}$ with cautious or malicious intention, we apply the proposed affine abstraction method to the uncertain functions \eqref{C_intention} and \eqref{M_intention}, respectively.

For {cautious driver} $(i=\text{C})$, the uncertain function \eqref{C_intention} can be rewritten as the following compact form:
\begin{align}
v_{y,o}(k+1) = G_C h_C(k),
\end{align}
where $G_C = \begin{bmatrix}- \delta t K_{p,C} & 1- \delta t K_{d,C}  & \delta t & \delta t \end{bmatrix} \in \mathbb{R}^{1\times4}$ and $h_C(k) = \begin{bmatrix} y_o(k) & v_{y,o}(k)  & w_y(k) & \tilde{d}_C(k) \end{bmatrix}^\mathsf{T} \in \mathbb{R}^{4}$. 
Using the proposed affine abstraction with state constraints and uncertain sets of intention parameters defined previously, two hyperplanes for the cautious intention are obtained as:
\begin{align*}
\overline{G}_C &= \begin{bmatrix} -0.27 & 0.175 & 0.3 & 0.3 \end{bmatrix}, \; \overline{b}_C = 12.285, \\
\underline{G}_C &= \begin{bmatrix} -0.27 & 0.175 & 0.3 & 0.3 \end{bmatrix}, \; \underline{b}_C = -12.285.
\end{align*}
As shown in Figure \ref{fig:C_result}, the obtained upper and lower hyperplanes over-approximate the uncertain linear dynamics with minimum approximation error.

%\begin{figure}[t!]
%\begin{center}
%		\includegraphics[scale=0.2]{C_result1.eps}
%		\includegraphics[scale=0.2]{C_result2.eps}
%		\caption{Affine abstraction of the uncertain dynamics of cautious driver?s velocity in $(y_o, v_{y,o})$ plane projection when $w_y(k) = -0.01$ and $\tilde{d}_C(k) = -0.392$ (\textbf{left}) and $w_y(k) = 0.01$ and $\tilde{d}_C(k) = 0.198$ (\textbf{left}).}
%	\end{center}
%\end{figure}

As illustrated in \eqref{M_intention}, all four state variables are involved in the function governing the other car's velocity with malicious intention.  The compact form of \eqref{M_intention} is given by
\begin{align}
v_{y,o}(k+1) = G_M h_M(k),
\end{align}
where $G_M = [ \delta t K_{p,M} \; \delta t K_{d,M} \; - \delta t K_{p,M} \; 1- \delta t K_{d,M}  \; \delta t \;  \delta t ] \in \mathbb{R}^{1 \times 6}$ and $h_C(k) = [x_e(k) \; v_{x,e}(k) \; y_o(k) \; v_{y,o}(k)  \; w_y(k) \;  \tilde{d}_C(k) ]^\mathsf{T} \in \mathbb{R}^{6}$. 
Using the same state domain and the uncertain sets, the affine abstraction for the malicious driver is obtained as:
\begin{align*}
\overline{G}_M &= \begin{bmatrix} 0.6 & 1.5 & -0.3 & 0.25 & 0.3 & 0.3 \end{bmatrix}, \; \overline{b}_M = 12.15, \\
\underline{G}_M &= \begin{bmatrix} 0 & 0 & -0.3 & 0.25 & 0.3 & 0.3 \end{bmatrix}, \; \underline{b}_M = -12.15.
\end{align*}
It is clear from Figure \ref{fig:M_result} that the obtained upper and lower hyperplanes envelop the uncertain dynamics in all projection planes. 
Moreover, the minimum approximation error is achieved when we project the uncertain dynamics and affine abstraction to $(y_{o}, v_{y,o})$ plane, as illustrated in Figure \ref{M_result6}.


%\newpage
%
%
%Here ego car inputs are $u$ and $v_{y,e}$ and the other car input is $d_{i}(k)$, where $i$ is the intention.\\
%state vector:
%\begin{align*}
%X = 
%\begin{bmatrix}
%x_{e}\\
%v_{x,e}\\
%y_{e}\\
%x_{o}\\
%v_{x,o}
%\end{bmatrix},
%U = 
%\begin{bmatrix}
%u(k)\\
%v_{y,e}(k)\\
%d_{i}
%\end{bmatrix}
%\end{align*}
%for Inattentive Model:
%\begin{align*}
%v_{x,o}(k+1) &= v_{x,o}(k) + d_{I}(k) \delta t
%\end{align*}
%for Malicious Model:
%\begin{align*}
%v_{x,o}(k+1) =& \,v_{x,o}(k) + (K_{d,M} \, (v_{x,e}(k)  -  v_{x,o}(k)) +\\
%& L_{p,M}(\overline{y} - y_{e}(k)) - L_{d,M} \, v_{y,e}(k) + d_{M}(k))\delta t
%\end{align*}
%Earlier, we had fixed $K_{d,M}$, $L_{d,M}$ and $L_{p,M}$. Now we have these with an uncertainty set. 
%For Cautious Model:
%\begin{align*}
%v_{x,o}(k+1) =& \,v_{x,o}(k) + (-K_{d,C} \, (v_{x,e}(k)  -  v_{x,o}(k)) -\\
%& L_{p,C}(\overline{y} - y_{e}(k)) + L_{d,C} \, v_{y,e}(k) + d_{C}(k))\delta t
%\end{align*}
%Note that the gains $L_{d,C}$ and $L_{d,M}$ have opposite signs, since the convention is that positive $y$ direction is perpendicular to the highway axis and away from the "other" car. \\
%For ease of notation, I am taking the Malicious Model and replacing the gains with a simple $K_{1}$, $K_{2}$ and $K_{3}$:
%\begin{align*}
%v_{x,o}(k+1) =& \,v_{x,o}(k) + (K_{1} \, (v_{x,e}(k)  -  v_{x,o}(k)) +\\
%& K_{2}(\overline{y} - y_{e}(k)) - K_{3} \, v_{y,e}(k) + d_{M}(k))\delta t
%\end{align*}
%Therefore:
%\begin{align*}
%X(k+1) =& 
%\begin{bmatrix}
%1 & \delta t & 0 & 0 & 0\\
%0 & 1 & 0 & 0 & 0\\
%0 & 0 & 1 & 0 & 0\\
%0 & 0 & 0 & 1 & \delta t\\
%0 & K_{1} \delta t & -K_{2} \delta t & 0 & 1 - K_{1} \delta t\\
%\end{bmatrix}
%X(k)\\
%&+\begin{bmatrix}
%0 & 0 & 0\\
%\delta t & 0 & 0\\
%0 & \delta t & 0\\
%0 & 0 & 0\\
%0 & -K_{3}\delta t & \delta t\\
%\end{bmatrix}
%U(k)
%+\begin{bmatrix}
%0\\
%0\\
%0\\
%0\\
%K_{2} \overline{y} \delta t
%\end{bmatrix}
%\end{align*}
%where $K_{n} \in [\underline{K}_{n},\overline{K}_{n}], \, n \in \{1,2,3\}$\\
%and $\forall k, X(k) \in \mathcal{X}$ and $U \in \mathcal{U}$ (each element of $X$ and $U$ vector lie in a defined range - so $\mathcal{X}$ and $\mathcal{U}$ are polytopes in 5 and 3 dimensions respectively.
%\\ \\
%There are two levels of robustification - \\
%1) w.r.t. matrices $A$, $B$ and $f$ (affine) i.e, w.r.t. the gains.\\
%2) w.r.t. $X$ and $U$.
%
%Now, we are looking for two matrices $\overline{A}$ and $\underline{A}$ such that:
%\begin{align*}
%&\underline{A} \, x(k) + \underline{B} \, u(k) + \underline{f} \leq A \, x(k) + B \, u(k) + f \\
%\leq &\overline{A} \, x(k) + \overline{B} \, u(k) + \overline{f}, \, \forall \, A \in  [A_{l},A_{u}], \forall x \in \{x:Q_{x} \, x \leq q_{x}\}\\
%& \forall u \in \{u:Q_{u} \, u \leq q_{u}\}
%\end{align*}
%\subsection{Robustifying the Gains}
%Taking one equality:
%\begin{align*}
%&A \, x(k) + B \, u(k) + f \leq \overline{A} \, x(k) + \overline{B} \, u(k) + \overline{f},\\
%&\, \forall \, A \in  [A_{l},A_{u}], \forall x \in \{x:Q \, x \leq q\}, \forall u \in \{u:Q_{u} \, u \leq q_{u}\} 
%\end{align*}

==> sec_preliminaries.tex <==
%!TEX root = main.tex
\section{Preliminaries}
\subsection{Notation}
For a vector $v \in \mathbb{R}^n$, $\|v\|_1$ denotes the vector $1$-norm .
%The $\text{vec}(\cdot)$ operator converts a matrix to a vector and is defined for matrix $M$ as: $\text{vec}(M) = \begin{bmatrix} M_1 & M_2 & \dots & M_p \end{bmatrix}^\mathsf{T}$, where $M_i$ represents the $i$th row of the matrix $M$.
An interval matrix $M^I$ is defined as a set of matrices of the form ${M}^I = [{M}_l, {M}_u] = \left\{ M \in \mathbb{R}^{n \times m} : {M}_l \le M \le {M}_u \right\}$, where ${M}_l$ and ${M}_u$ are $n \times m$ matrices, and the inequality is to be understood componentwise. 
If $A$ is a interval matrix with elements $[{a}_{l,ij}, {a}_{u,ij}]$ and $B$ is a matrix with real elements $b_{ij}$ such that $b_{ij} \in [{a}_{l,ij}, {a}_{u,ij}]$ for all $i$ and $j$, then we write $B \in A$.
We denote $[n]$ as the initial segment $1, \ldots, n$ of the natural numbers, and $|\mathcal{X} |$ as the cardinality of a set $\mathcal{X}$,  and $I_n$ as a $n \times n$ identity matrix, respectively.

\subsection{Modeling Framework}
Consider an uncertain affine discrete-time system: % of the form:
\begin{align}
x& (k+  1) =  {A}  x(k) + {B}_u u(k) + {B}_w w(k) + {B}_f f,  \label{dynamics}
\end{align}
where $x(k) \in \mathcal{X} \subset \mathbb{R}^{n}$ is the system state, $u(k) \in \mathcal{U} \subset \mathbb{R}^{m}$ is the control input, and $w(k) \in \mathcal{W} \subset  \mathbb{R}^{m_w}$ is the process noise at the current time instant $k$, the vector $f \in \mathcal{F} \subset  \mathbb{R}^{m_f}$ is an unknown additive constant. Throughout the paper, we assume that the domain $\mathcal{X}$, $\mathcal{U}$, $\mathcal{W}$ and $\mathcal{F}$ are polyhedral sets:% defined as 
\begin{subequations} \label{constr}
\begin{gather}
\mathcal{X} = \left \{  x \in \mathbb{R}^{n} : Q_x x \le q_x\right \},  \label{constr_x}\\
\mathcal{U} = \left \{ u \in \mathbb{R}^{m} : Q_u u \le q_u\right \}, \label{constr_u}\\
\mathcal{W} = \left \{  w \in \mathbb{R}^{m_w} : Q_w w \le q_w\right \}, \label{constr_w}\\
\mathcal{F} = \left \{  f \in \mathbb{R}^{m_f} : Q_f f \le q_f\right \},  \label{constr_f}
\end{gather}
 \end{subequations}
 where the matrices $Q_x \in \mathbb{R}^{k_x \times n}$, $Q_u \in \mathbb{R}^{k_u \times m}$, $Q_w \in \mathbb{R}^{k_w \times m_w}$, $Q_f \in \mathbb{R}^{k_f \times n}$, and the vectors $q_x \in \mathbb{R}^{k_x}$, $q_u \in \mathbb{R}^{k_u}$, $q_w \in \mathbb{R}^{k_w}$ and $q_f \in \mathbb{R}^{k_f}$ are constant and imposed to describe physical constraints or by the desired domain of operation/observation. 
Due to measurement errors or component tolerances, the state matrix $A \in \mathbb{R}^{n \times n}$, input matrix $B \in \mathbb{R}^{n \times m}$, noise matrix $B_w \in \mathbb{R}^{n \times m_w}$, and fault matrix $B_f \in \mathbb{R}^{n \times m_f}$ are uncertain and known to the extent of  
\begin{subequations} \label{interval_matrix}
\begin{gather}
A \in A^{I} = [{A}_l, {A}_u], 
B \in B^{I} = [{B}_l, {B}_u],   \\
B_w \in B^{I}_w = [{B}_{w,l}, {B}_{w,u}], 
B_f \in B^{I}_f = [{B}_{f,l}, {B}_{f,u}], 
\end{gather}
\end{subequations}
where the interval matrices or vectors $A^{I}$, $B^{I}$, $B_w^{I}$ and $B_f^{I}$ define the ranges of the uncertainties. 

Consequently, for compactness, the uncertain linear discrete-time system \eqref{dynamics} is further rewritten as 
\begin{align} \label{augment_dynamics}
x(k+1) = G h(k), 
\end{align}
where the augmented state $h (k) = \begin{bmatrix} x^\mathsf{T}(k)& u^\mathsf{T}(k)& w^\mathsf{T}(k)& f ^\mathsf{T}\end{bmatrix}^\mathsf{T} \in \mathbb{R}^{\xi}$ and the augmented uncertain system matrix $G = \begin{bmatrix} A  & B & B_w & B_f \end{bmatrix} \in \mathbb{R}^{n \times {\xi}}$ with $\xi = n+m+m_w+m_f$. In view of \eqref{constr}, it is clear that $h(k) \in \mathcal{H} \subset \mathbb{R}^{\xi}$, which is also a polyhedral set given as 
\begin{align} \label{augment_constr}
\mathcal{H} = \left \{  h \in \mathbb{R}^{\xi} : Q h \le q \right \},
\end{align}
where $Q= \text{diag}(Q_x,Q_u,Q_w,Q_f) \in \mathbb{R}^{k \times \xi}$, $q = \begin{bmatrix} q^\mathsf{T}_x  & q^\mathsf{T}_u & q^\mathsf{T}_w & q^\mathsf{T}_f \end{bmatrix}^\mathsf{T} \in \mathbb{R}^{k}$
and $k = k_x+k_u+k_w+k_f$.
Moreover, considering the system uncertainties defined by interval matrices in \eqref{interval_matrix}, the augmented system matrix $G$ satisfies
\begin{align} \label{augment_interval_matrix}
G \in G^I = [{G}_l, {G}_u], 
\end{align}
where ${G}_l = \begin{bmatrix} {A}_l & {B}_l & {B}_{w,l} & {B}_{f,l} \end{bmatrix} \in \mathbb{R}^{n \times \xi}$ and ${G}_u = \begin{bmatrix} {A}_u & {B}_u & {B}_{w,u} & {B}_{f,u} \end{bmatrix} \in \mathbb{R}^{n \times \xi}$.

\subsection{Problem Statement}
In this paper, we aim to over-approximate/abstract the uncertain affine discrete-time dynamics by a pair of affine hyperplanes ($\underline{f}$, $\overline{f}$) such that for all $G \in G^I$ and $h(k) \in \mathcal{H}$, we have that $\underline{f} \le G h(k) \le \overline{f}$ (i.e., $G h(k)
$ is lower and upper bounded by $\underline{f}$ and $\overline{f}$). As a result, the uncertain affine system defined in \eqref{dynamics} lies between the lower and upper affine hyperplanes, which are defined as 
\begin{align} \label{hyper_plane}
\underline{f}(h(k)) = \underline{G} h(k) + \underline{b},  \;
\overline{f}(h(k)) = \overline{G} h(k) + \overline{b},
\end{align}
where the matrices $\underline{G}$ and $\overline{G}$, and the vectors $\underline{b}$ and $\overline{b}$ are constant and of appropriate dimensions. 
We say that an affine plane pair ($\underline{f}$, $\overline{f}$) over-approximates/abstracts the uncertain affine dynamics if $\underline{f}\left( h(k) \right) \le G h(k) \le \overline{f}\left( h(k) \right)$, $\forall \, G \in G^I$ and $\forall \, h(k) \in \mathcal{H}$. The affine hyperplanes pair ($\underline{f}$, $\overline{f}$) is then the affine abstraction of the uncertain affine dynamics.

\begin{definition}[Approximation Error] \label{approx}
If a pair of affine hyperplanes $(\underline{f}, \overline{f})$ over-approximates an uncertain affine discrete-time dynamics defined in \eqref{augment_dynamics} over the system constraints $h(k)\in\mathcal{H}$ and uncertainties $G \in G^I$, then the approximation error of the abstraction with respect to the uncertain affine dynamics is defined as
\begin{align}
e(\underline{f}, \overline{f}) = \max_{h(k) \in \mathcal{H}} \|\overline{f} \left( h(k) \right) - \underline{f} \left( h(k) \right)\|_1. 
\end{align}
\end{definition}

\begin{problem}[Affine Abstraction] \label{problem1}
For an uncertain affine discrete-time dynamics given in \eqref{augment_dynamics} with the polyhedral domain $h(k)\in\mathcal{H}$ and the uncertain system matrices $G \in G^I$, the affine abstraction is to find an affine hyperplane pair ($\underline{f}$, $\overline{f}$) (i.e., the lower and upper hyperplanes defined in \eqref{hyper_plane}) to over-approximate/abstract the given uncertain affine dynamics with the minimum approximation error.
Thus, the affine abstraction problem for uncertain linear discrete-time systems is equivalent to a robust optimization problem:
\begin{subequations} \label{p1}
\begin{align} 
\notag \underset{\theta, \overline{G}, \underline{G}, \overline{b}, \underline{b}}{\text{min}} \quad &\theta   \\  
\text{s.t.} \hspace{0.7cm} 
& \hspace{-0.1cm}  \begin{array}{l} \label{p1:a}   
\overline{G} \, {h}(k) + \overline{b}  \geq G {h}(k) , \\ \vspace{-0.1cm}
\quad \forall \,G \in G^I, \forall \, h(k) \in \mathcal{H},  
\end{array} \\ 
& \hspace{-0.1cm}   \begin{array}{l} \label{p1:b}
\underline{G} \, {h}(k) + \underline{b}  \leq G {h}(k),  \\ \vspace{-0.1cm}
\quad \forall \,G \in G^I, \forall \, h(k) \in \mathcal{H}, 
\end{array} \\
& \hspace{-0.1cm}  \max_{h(k) \in \mathcal{H}} \|\overline{f} \left( h(k) \right)- \underline{f}\left( h(k) \right) \|_1 \le \theta , \label{p1:c} 
%(\overline{G} - \underline{G}) \, {h}(k) +(\overline{b} - \underline{b}) \leq \theta, \\
\end{align}
\end{subequations}
where $\theta$ is the least upper bound on the approximation error.
\end{problem}






==> sec_result2_v2.tex <==
%!TEX root = main.tex
\subsection {Data-Driven Model Invalidation Algorithm}
%In order to achieve model discrimination, i.e., only one model will not be invalidated, %solve Problem \ref{problem1}, 
%we will assume the following: % to ensure that two models are inconsistent for length-$T$ trajectory:
%\begin{assumption} \label{assumption1}
%The length-$T$ output trajectories are only consistent with one unknown model. Thus, we must have $\mathcal{B}^T(\mathcal{G}) \cap \mathcal{B}^T(\mathcal{G}') =\emptyset$ for all $\mathcal{G} \neq \mathcal{G}'$. %, where $\mathcal{G}$ is original model and $\mathcal{G}'$ is the model to be invalidated.
%%There exist and only exist one valid model 
%%$\mathcal{G}_i$, i.e., $\mathcal{G}_j$. % in the system.
%\end{assumption}
% \moh{SOME JUSTIFICATION FOR ASSUMPTION}
 % \begin{lemma} \label{lemma_formulation}
 % Given the partition of the space, the piecewise constraint: $x_{k+1}\leq$
 % \end{lemma}
 
 We apply an optimization-based model invalidation approach to determine if the data-driven abstraction obtained in the previous section is incompatible with new observed length-$T$ output trajectory. %Since we assume that only one original unknown model can be consistent, with a sufficiently accurate abstraction, where enough data is sampled according to Proposition \ref{Abs}, we can also assume that the length-$T$ output trajectory is only compatible with the abstracted model. Using this fact, 
In particular, we propose the following model invalidation algorithm that (in)validates the abstraction model $\mathcal{H}$:

% \vspace{-0.1cm}
% Given an abstracted model $\mathcal{H}$ and a length-$T$ output sequence $\{\tilde{y}_k\}_{k=0}^{k=T-1}$, the model is invalidated if the following problem is infeasible:
% \begin{subequations} \label{MI_o}
% \begin{align} \tag{MI}
% \nonumber & \hspace{-0.3cm} \text{Find} \ {y_k}, w_k, v_k\ \forall  k  \in\mathbb{Z}_{T-1}^0         \\[-0.2em]
% \nonumber &\hspace{-0.3cm} \text{subject to} \  \forall  k  \in\mathbb{Z}_{T-1}^{n_y}: \\
% & \hspace{0.5cm} y_{k+1} \leq \overline{f}(s_k) +w_k,\label{constraint_1}\\[-0.2em]
% & \hspace{0.5cm} y_{k+1} \geq \underline{f}(s_k) +w_k,\label{constraint_2}\\[-0.2em]
% % & \hspace{0.5cm} S_ix_k +T_iu_k\leq \beta_i + s_{i,k} \mathds{1}_{c_i}, \label{constraint_3}\\[-0.2em]
%  \nonumber & \hspace{0.5cm} \forall k \in \mathbb{Z}_{T-1}^0:  \\[-0.2em]
%  & \hspace{0.5cm} \tilde{y}_k = y_k+v_k, \ \underline{y}_k \leq y_k \leq \overline{y}_k,\\ 
%    & \hspace{0.5cm}-\varepsilon_w \mathbbm{1}\leq w_k\leq \varepsilon_w \mathbbm{1}, -\varepsilon_v \mathbbm{1}\leq v_k\leq \varepsilon_v \mathbbm{1},
%  % & \hspace{0.5cm}   \\[-0.2em]
%%   & \hspace{0.5cm} ||w_k||\leq \varepsilon_w, \ ||v_k||\leq \varepsilon_v,
% % &\hspace{.5cm}  a_{i,k}\in\{0, 1\}, \ \textstyle\sum_{i\in[p]} a_{i,k}=1, \label{constraint_sos1}\\[-0.2em] 
% % & \hspace{0.5cm} ||\omega_k||\leq \varepsilon_\omega, \ ||v_k||\leq \varepsilon_v, \ (a_{i,k}, s_{i,k}):SOS\text{-}1,
% \end{align}
% \end{subequations}
% where $s_k=[y_k,\cdots,y_{k-n_y+1}]^T$, $\underline{y}_k$ and $\overline{y}_k$ are given bounds of $y_k$. 
 
% Through the following Theorem \ref{theorem2}, we will show
\begin{theorem} \label{theorem2}
Given an abstracted model $\mathcal{H}$ and a length-$T$ output sequence $\{\tilde{y}_k\}_{k=0}^{k=T-1}$, the data-driven model invalidation problem in Problem 1.\ref{problem1.2} is equivalent to the following feasibility problem:
 \begin{subequations}
 \begin{align}
 \nonumber & \hspace{-0.3cm} \text{Find} \ {y_k}, w_k, v_k \ \forall  k  \in\mathbb{Z}_{T-1}^0         \\[-0.em]
 \nonumber &\hspace{-0.3cm} \text{subject to} \  \forall  k  \in\mathbb{Z}_{T-1}^{n_y}, \forall  \ell  \in\mathbb{Z}_{N}^{1}, \forall (\tilde{s}^o_{j,\ell},\tilde{y}^o_{j+1,\ell})\in \overline{\mathcal{D}}_\ell: \\
 & \hspace{0.3cm} y_{k+1} \leq \tilde{y}^o_{j+1, \ell}+L_p||s_k-\tilde{s}^o_{j, \ell}||_p +\varepsilon_t+w_k, \label{constraint1'}\\[-0.em] %\ \forall (\tilde{s}^o_j,\tilde{y}^0_{j+1})\in \overline{\mathcal{D}}, \\[-0.2em]
 & \hspace{0.3cm} y_{k+1} \geq \tilde{y}^o_{j+1, \ell}-L_p||s_k-\tilde{s}^o_{j, \ell}||_p -\varepsilon_t+w_k, \label{constraint2'}\\[-0.em] %\ \forall (\tilde{s}^o_j,\tilde{y}^0_{j+1})\in \overline{\mathcal{D}}, \label{constraint2'}\\[-0.2em]
 % & \hspace{0.5cm} S_ix_k +T_iu_k\leq \beta_i + s_{i,k} \mathds{1}_{c_i}, \label{constraint_3}\\[-0.2em]
   \nonumber & \hspace{0.3cm} \forall k \in \mathbb{Z}_{T-1}^0:  \\[-0.em]
  & \hspace{0.3cm} \tilde{y}_k = y_k+v_k, \ \underline{y}_k \leq y_k \leq \overline{y}_k,\\ 
    & \hspace{0.3cm}-\varepsilon_w \mathbbm{1}\leq w_k\leq \varepsilon_w \mathbbm{1}, -\varepsilon_v \mathbbm{1}\leq v_k\leq \varepsilon_v \mathbbm{1},% \\[-0.2em]
  % & \hspace{0.3cm} \underline{x}_k \leq x_k \leq \overline{x}_k,  \\[-0.2em]
%   & \hspace{0.3cm} ||w_k||\leq \varepsilon_w, \ ||v_k||\leq \varepsilon_v,
 % &\hspace{.5cm}  a_{i,k}\in\{0, 1\}, \ \textstyle\sum_{i\in[p]} a_{i,k}=1, \label{constraint_sos1}\\[-0.2em] 
 % & \hspace{0.5cm} ||\omega_k||\leq \varepsilon_\omega, \ ||v_k||\leq \varepsilon_v, \ (a_{i,k}, s_{i,k}):SOS\text{-}1,
 \end{align}
 \end{subequations}
 where $\overline{\mathcal{D}_\ell} = \{(\tilde{s}^o_{j,\ell}, \tilde{y}^o_{j+1, \ell})|j=n_y, \cdots, T_\ell-1\}$ is one trajectory of $\overline{\mathcal{D}}$ and  $\overline{\mathcal{D}}=\bigcup_{\ell=1}^N \overline{\mathcal{D}}_\ell$ is the given sampled data set from which we obtain a data-driven abstraction $\mathcal{H}$ with $\underline{y}_k$ and $\overline{y}_k$ as given bounds of $y_k$, $s_k=[y_k,\cdots,y_{k-n_y+1}]^T$, $\underline{y}_k$, $\varepsilon_t=[\varepsilon_t^{(1)}, \hdots, \varepsilon_t^{(m)}]^\top$ and $L_p=[L_p^{(1)}, \hdots, L_p^{(m)}]^\top$.
\end{theorem}
% \vspace{-0.35cm}
\begin{proof}
By the definition of model invalidation for abstracted model $\mathcal{H}$, we know that 
%Given an abstracted model $\mathcal{H}$ and a length-$T$ output sequence $\{\tilde{y}_k\}_{k=0}^{k=T-1}$, 
the abstraction  is invalidated if the following problem is infeasible:
 \begin{subequations} \label{MI_o}
 \begin{align} \tag{MI}
 \nonumber & \hspace{-0.3cm} \text{Find} \ {y_k}, w_k, v_k\ \forall  k  \in\mathbb{Z}_{T-1}^0         \\[-0.em]
 \nonumber &\hspace{-0.3cm} \text{subject to} \  \forall  k  \in\mathbb{Z}_{T-1}^{n_y}: \\
 & \hspace{0.5cm} y_{k+1} \leq \overline{f}(s_k) +w_k,\label{constraint_1}\\[-0.em]
 & \hspace{0.5cm} y_{k+1} \geq \underline{f}(s_k) +w_k,\label{constraint_2}\\[-0.em]
 % & \hspace{0.5cm} S_ix_k +T_iu_k\leq \beta_i + s_{i,k} \mathds{1}_{c_i}, \label{constraint_3}\\[-0.2em]
  \nonumber & \hspace{0.5cm} \forall k \in \mathbb{Z}_{T-1}^0:  \\[-0.em]
  & \hspace{0.5cm} \tilde{y}_k = y_k+v_k, \ \underline{y}_k \leq y_k \leq \overline{y}_k,\\ 
    & \hspace{0.5cm}-\varepsilon_w \mathbbm{1}\leq w_k\leq \varepsilon_w \mathbbm{1}, -\varepsilon_v \mathbbm{1}\leq v_k\leq \varepsilon_v \mathbbm{1}.
  % & \hspace{0.5cm}   \\[-0.2em]
%   & \hspace{0.5cm} ||w_k||\leq \varepsilon_w, \ ||v_k||\leq \varepsilon_v,
 % &\hspace{.5cm}  a_{i,k}\in\{0, 1\}, \ \textstyle\sum_{i\in[p]} a_{i,k}=1, \label{constraint_sos1}\\[-0.2em] 
 % & \hspace{0.5cm} ||\omega_k||\leq \varepsilon_\omega, \ ||v_k||\leq \varepsilon_v, \ (a_{i,k}, s_{i,k}):SOS\text{-}1,
 \end{align}
 \end{subequations}
% where $s_k=[y_k,\cdots,y_{k-n_y+1}]^T$, $\underline{y}_k$ and $\overline{y}_k$ are given bounds of $y_k$. 
 
Since the upper bound of the abstraction is given by \eqref{upper_func}, constraint \eqref{constraint_1} is equivalent to \eqref{constraint1'}. %$x_{k+1} \leq \tilde{y}_j+L_p||\tilde{s}_j-s_k||_p,\ \forall (\tilde{s}_j,\tilde{y}_j)\in\mathcal{D}$. 
Similarly, by \eqref{lower_func}, the \eqref{constraint2'} is equivalent to \eqref{constraint_2}. Thus, two optimization problems are equivalent. If the above optimization problem is infeasible, it means that the output sequence $\{\tilde{y}_k\}_{k=0}^{k=T-1}$ cannot be consistent with the length-$T$ behavior of $\mathcal{H}$, i.e., $\{\tilde{y}_k\}_{k=0}^{k=T-1} \notin \mathcal{B}^T(\mathcal{H})$, hence the model is invalidated.
\end{proof}
From Corollary \ref{linear}, by choosing the suitable vector norm, i.e., $p=1$ or $\infty$, the optimization problem in Theorem \ref{theorem2} is a linear programming/feasibility problem. 

\begin{remark}\label{rem:1} By Proposition \ref{Abs}, we could choose to only use a strict subset of the sampled data, $\overline{\mathcal{D}}_{\ell} (\tilde{y}_k)\subseteq \overline{\mathcal{D}}_\ell$, without violating the guarantees of Theorem \ref{theorem2}, where $\overline{\mathcal{D}}_{\ell} (\tilde{y}_k)$ may be a function of the new observed data $\tilde{y}_k$. In this case, we will replace \eqref{constraint1'} and \eqref{constraint2'} with the following constraints:
\begin{align*}
y_{k+1} \leq \tilde{y}^0_{j+1,\ell,k}+L_p||s_k-\tilde{s}^o_{j,\ell,k}||_p +\varepsilon_t+w_k,\\
y_{k+1} \geq \tilde{y}^0_{j+1,\ell,k}-L_p||s_k-\tilde{s}^o_{j,\ell,k}||_p -\varepsilon_t+w_k,
\end{align*}
for all $(\tilde{s}^o_{j,\ell,k},\tilde{y}^0_{j+1,\ell,k}) \in \overline{\mathcal{D}}_{\ell} (\tilde{y}_k)$. 
The advantage of this ``downsampling" is that the computational time can be reduced but at the cost of the abstracted model precision and thus the ability of the data-driven model invalidation algorithm to eliminate inconsistent models. We will explore this downsampling strategy in the simulation section.
\end{remark}

\subsection{Estimation of Lipschitz Constant}
In the previous sections, the Lipschitz constants are assumed to be given. However, they may be also unknown in some cases. In this case, we will adopt the approach in \cite{calliess2014conservative} to estimate the Lipschitz constant from sampled data set $\overline{\mathcal{D}}=\{(\tilde{s}^o_j, \tilde{y}^o_{j+1})|j=n_y, \cdots, N-1\}$ that is corrupted by bounded noise:
% \begin{align}
% L_p = \max_{i\neq j} \frac{|y^i -y^j|}{|s^i-s^j|_p}.
% \end{align}
% For the data set $\mathcal{D}=\{(\tilde{s}^i, \tilde{y}^i)|i=1,2 \cdots, N\}$ corrupted by bounded noise, the constant can be estimated with following equation:
\begin{align} \label{estimateL}
\hat{L}^{(i)}_p = \max_{j\neq k} \frac{|(\tilde{y}^o_j)^{(i)} -(\tilde{y}^o_k)^{(i)}_k|-2\varepsilon_v}{||\tilde{s}^o_j-\tilde{s}^o_k||_p+2\varepsilon_s}.
\end{align}

Since the accuracy of $L^{(i)}_p$ is crucial for the results in the previous section, we proceed to find some guarantees that we obtain the right estimate with high probability. To achieve this, we leverage a classical result on probably approximately correct (PAC) learning for linear separators, which is summarized below:
\begin{definition}[Linear Separators\cite{kearns1994introduction}] \label{def:linear} For $\Gamma \subset \mathbb{R} \times \mathbb{R}$, a linear separator is a pair $(a, b)\in \mathbb{R}^2$ such that
\begin{align} \label{eq:linsep}
\forall(x, y) \in \Gamma: \ x \leq ay +b.
\end{align}
\end{definition}

\begin{proposition}[PAC Learning \cite{kearns1994introduction}] 
Let $\epsilon, \delta \in \mathbb{R}^+$. If number of sampling points is $N\geq\frac{1}{\epsilon}\ln\frac{1}{\delta}$, where the sample points $\Gamma$  are drawn from a distribution $\mathcal{P}$, then, with probability greater than $1 - \delta$, a linear separator $(a,b)$ has an error $\texttt{err}_{\mathcal{P}}$ of less than $\epsilon$, where the error of a pair $(a, b)$ is defined as $\texttt{err}_{\mathcal{P}}(a,b)=\mathcal{P}({(x,y)\in\Gamma|x>ay+b})$.
\end{proposition}
%\begin{proof}
%The detailed proof can be found in \cite{kearns1994introduction}.
%\end{proof}

%To find some linear separators $(a, b)$ for $\Gamma$ by sampling points in $\Gamma$, we assume that points of $\Gamma$ can be drawn by some unknown distribution $Distr$. The error of a pair $(a, b)$ is defined to be $\texttt{err}_{Distr}(a,b)=Distr({(x,y)\in\Gamma|x>ay+b})$ where $Distr(X)$ is the measure of points that $(a,b)$ violates linear separator under distribution $Distr$. The algorithm to find $(a,b)$ is given by Algorithm \ref{Alg1}. Then the following result hold according to PAC learning theory,

%\begin{algorithm}[b] 
%\SetAlgoLined\DontPrintSemicolon \small
%% \KwData{$\tt{Models} \  \mathit{\mathcal{G}_1 \ \dots \mathcal{G}_{N_f}}$, $\tt{Input\text{-}}\tt{Output} \ \tt{Sequence} =  \mathit{\{u_\ell, y_\ell\}_{\ell=0}^{\ell=k-1}}$} 
%\SetKwFunction{findmodel}{findPair}
%% \SetKwFunction{check}{checkValid}
%\SetKwProg{func}{function}{}{}
%\func{\findmodel{$\Gamma$, $Distr$, $N$}}
%{
%  % $\tt{valid} \leftarrow  \mathit{[N_f]} $\\
%  % \For{$i=1:N_f$} {
%  % Check Feasibility of Theorem \ref{theorem2} \\
%  % \If{infeasible} 
%  % {
%  %   Remove $i$ from $\tt{valid}$
%  %   }
%  % }
%  Draw $N$ pairs of data $(\tilde{s}_1, \tilde{y}_1), (\tilde{s}_2,\tilde{y}_2),\cdots,(\tilde{s}_N,\tilde{y}_N)$ from $\Gamma'$ based on distribution $Distr'$ \\
%  Transfer $N$ pairs of data to $\frac{N(N-1)}{2}$ pairs of data, $(||\tilde{s}_i-\tilde{s}_j||_p+2\varepsilon_w, |\tilde{y}_i-\tilde{y}_j|-2\epsilon_v) \ \forall \ i\neq j, \ i,\ j \in \{1,2,\cdots, N\}$\\
%  Find $\tilde{L_p}$ $s.t.\ \tilde{L_p}(||\tilde{s}_i-\tilde{s}_j||_p+2\varepsilon_w) \leq |\tilde{y}_i-\tilde{y}_j|-2\epsilon_v \ \forall \ i\neq j, \ i,\ j \in \{1,2,\cdots, N\} $ \\
%  \KwRet{$\tilde{L_p}$}
%}
%% \func{\check{$\mathcal{G}, \{u_k, y_k\}_{k=0}^{k=t}$}}
%% {
%%   Refer to Theorem \ref{theorem2} for its description \\
%%   \KwRet{$\tt{ifValid}$}
%% }
%  \caption{Lipschitz Constant Estimation}%: find pair $(a,b)$}
%  \label{Alg1}
%\end{algorithm}\normalsize


From Definition \ref{def:linear}, it is easy to verify that our estimate of $\hat{L}_P^{(i)}$ \eqref{estimateL} is a special case of the linear separator \eqref{eq:linsep}, with $b=0$. Thus, the estimated $\hat{L}_P^{(i)}$ using \eqref{estimateL} is guaranteed with high probability to be close to the true Lipschitz constant of the original unknown function if we have sufficient data. %from Equation \eqref{estimateL} can be ensured to work for future abstraction with high probability.

==> sec_result_v2.tex <==
%!TEX root = main.tex
\section {Data-driven Abstraction and Model Invalidation}
In this section, we first introduce an approach for obtaining a data-driven abstraction of the unknown system \eqref{eq:system}, before proposing an optimization-based approach to (in)validate the resulting abstraction model with given new noisy output trajectories. The two algorithms we propose solve Problem 1.\ref{problem1.1} and 1.\ref{problem1.2}, and consequently, Problem \ref{problem1} by Proposition \ref{propMI}.
\subsection {Data-Driven Abstraction Algorithm} %\jin{ref to add}}{}
\begin{theorem} \label{LipschitzInterpolation}{}
Consider system \eqref{eq:system} and its corresponding data set $\overline{\mathcal{D}}=\bigcup_{\ell=1}^N\{(\tilde{s}^o_{j,\ell}, \tilde{y}^o_{j+1,\ell})|\moh{j}=n_y, \cdots, T_\ell-1\}$. \moh{Suppose Assumption \ref{assumption:lip} holds. Then, for all $s\in \mathcal{S}$, $\underline{f}(\cdot)$ and $\overline{f}(\cdot)$ are lower and upper abstraction functions for unknown function $f(\cdot)$, i.e., $\forall s \in \mathcal{S}$, $\underline{f}(s) \leq f(s) \leq \overline{f}(s)$,  where $\underline{f}(\cdot) \triangleq \begin{bmatrix}\underline{f}^1(\cdot) & \dots & \underline{f}^i(\cdot) & \dots & \underline{f}^m(\cdot) \end{bmatrix}^\top$, $\overline{f}(\cdot) \triangleq \begin{bmatrix}\overline{f}^1(\cdot) & \dots & \overline{f}^i(\cdot) & \dots & \overline{f}^m(\cdot) \end{bmatrix}^\top$ and} %from system dynamic function \eqref{eq:system} and Lipschitz constant $L_p$ of the function, the abstraction of the function $f$ is following:
 \begin{subequations}
 \begin{align} %\label{eq:bounds}
% \overline{f}(s) = \min_{i=1,2,\codts,N}y_i+L_p|s-s_i|_p 
% & \underline{f}(s) = \max_{i=1,2,\codts,N}y_i-L_p|s-s_i|_p \\[-0.2em] is 
& \overline{f}\moh{^i}(s) \hspace{-0.05cm}= \hspace{-0.25cm} \min_{\substack{j \in \{n_y,\hdots, T_\ell-1\},\\ \ell \in \{1,\hdots,N\}}} \hspace{-0.1cm} ((\tilde{y}^o_{j+1,\ell})^{(i)}\hspace{-0.1cm}+\hspace{-0.1cm}L^{(i)}_p\|s\hspace{-0.1cm}-\hspace{-0.1cm}\tilde{s}^o_{j,\ell}\|_p)\hspace{-0.1cm}+\hspace{-0.1cm}\varepsilon^{(i)}_{t} \hspace{-0.05cm}, \label{upper_func}\\[-0.2em]
 & \underline{f}\moh{^i}(s)  \hspace{-0.05cm}= \hspace{-0.25cm}\max_{\substack{j \in \{n_y,\hdots, T_\ell-1\},\\ \ell \in \{1,\hdots,N\}}}\hspace{-0.1cm} ((\tilde{y}^o_{j+1,\ell})^{(i)}\hspace{-0.1cm}-\hspace{-0.1cm}L^{(i)}_p\|s\hspace{-0.1cm}-\hspace{-0.1cm}\tilde{s}^o_{j,\ell}\|_p) \hspace{-0.1cm}-\hspace{-0.1cm}\varepsilon^{(i)}_{t} \hspace{-0.05cm}, \label{lower_func}
 \end{align}
 with $\varepsilon^{(i)}_t \triangleq \varepsilon^{(i)}_w+\varepsilon^{(i)}_v+L^{(i)}_p\varepsilon_s$, \moh{for all $i \in \{1\dots m \}$.  Moreover, $\underline{f}^i$ and $\overline{f}^i$ are $L^{(i)}_p$-Lipschitz functions and $\underline{f}$ and $\overline{f}$ are also Lipschitz continuous.}
 \end{subequations}
\end{theorem}
\begin{proof}
It follows from Assumption \ref{assumption:lip} that
$$|f^i(x_2)-f^i(x_1)| \leq L^{(i)}_p\|x_2-x_1\|_p, \forall i \in \{1\dots m\}.$$
Let $x_2=s$ be the generic variable and $x_1=s^o_{j,\ell}=\tilde{s}^o_{j,\ell}-z^o_{j,\ell}$ be the de-noised observation of the noisy $\tilde{s}^o_{j,\ell}$, where $z^o_{j,\ell}$ satisfies $\|z^o_{j,\ell}\|_p \leq \varepsilon_s$. Furthermore, from \eqref{eq:system} and \eqref{eq:output}, we have $f^i(s^o_{j,\ell})=(y^o_{j+1,\ell})^{(i)}-(w^o_{j,\ell})^{(i)}=(\tilde{y}^o_{j+1,\ell})^{(i)}-(w^o_{j,\ell})^{(i)}-(v^o_{j,\ell})^{(i)}$.

Next, applying the triangle inequality to 
% \begin{gather*}(\tilde{y}^o_{j+1})^{(i)}-(w_j^o)^{(i)}-(v^o_j)^{(i)}-L^{(i)}_p\|s-\tilde{s}^o_{j,\ell}-z^o_j\|_p \\  \leq  f(s) \leq (\tilde{y}^o_{j+1,\ell})^{(i)} \hspace{-0.05cm}-\hspace{-0.05cm}(w_{j,\ell}^o)^{(i)}\hspace{-0.05cm}-\hspace{-0.05cm}(v^o_{j,\ell})^{(i)}\hspace{-0.05cm}+\hspace{-0.05cm}L^{(i)}_p\|s-\tilde{s}^o_{j,\ell}-z^o_{j,\ell}\|_p,\end{gather*}
\hspace{-0.3cm}\begin{gather*}(\tilde{y}^o_{j+1,\ell})^{(i)}-(w_{j,\ell}^o)^{(i)}-(v^o_{j,\ell})^{(i)}-L^{(i)}_p\|s-\tilde{s}^o_{j,\ell}-z^o_{j,\ell}\|_p \leq \\ \hspace{-0.3cm} f(s) \leq (\tilde{y}^o_{j+1,\ell})^{(i)} \hspace{-0.05cm}-\hspace{-0.05cm}(w_{j,\ell}^o)^{(i)}\hspace{-0.05cm}-\hspace{-0.05cm}(v^o_{j,\ell})^{(i)}\hspace{-0.05cm}+\hspace{-0.05cm}L^{(i)}_p\|s-\tilde{s}^o_{j,\ell}-z^o_{j,\ell}\|_p,\end{gather*}
%and triangle inequality that $\forall (\tilde{s}^o_j,\tilde{y}^o_j) \in \overline{\mathcal{D}},j \in \{1\dots m\}, i \in \{1\dots m\}, \forall s \in \mathcal{S}$, $\forall w^{(i)}_j,v_j \ s.t. \ |w^{(i)}_j| \leq \varepsilon^{(i)}_w,\|v_j\|_p \leq \varepsilon_v$, $|f^i(s)-\tilde{y}^{(i)}_j-w^{(i)}_j|=|f^i({s})-{y}^{(i)}_j| \leq L^{(i)}_p\|{s}-{s}_j\|_2  \leq L^{(i)}_p \|s-\tilde{s}_j\|_p$. This implies that $\tilde{y}^{(i)}_j+w^{(i)}_j-L^{(i)}_p\|s-\tilde{s}_j-v_j\|_p \leq f(s) \leq \tilde{y}^{(i)}_j+w^{(i)}_j+L^{(i)}_p\|s-\tilde{s}_j-v_j\|_p$. 
the results in \eqref{upper_func} and \eqref{lower_func} follow from the fact that these inequalities should hold for \emph{all} the sampled data and \emph{all} the possible values of noise signals. $L^{(i)}_p$-Lipschitz continuity of upper and lower abstraction functions is implied by the fact that function $\|.\|_p$ is $1$-Lipschitz continuous and \cite{sukharev1978optimal}.  
%\begin{align}
%\max_{j \in \{1\dots N\}} (\tilde{y}_j-L^i_p\|s-\tilde{s}_j\|_p)-\varepsilon_{s} \leq \min_{j \in \{1\dots N\}} (\tilde{y}_j+L^i_p\|s-\tilde{s}_j\|_p)+\varepsilon_{s}
%\end{align}
\end{proof}
\begin{corollary} \label{linear}
 \moh{If $1$ or $\infty$} norm \moh{is considered, i.e., $p=1$ or $\infty$, then} the abstraction \moh{functions are} piecewise affine function\moh{s}, and the corresponding abstraction is called a piecewise affine abstraction.
\end{corollary}
\begin{proposition} \label{Abs}
\moh{The abstraction approach described in Theorem \ref{LipschitzInterpolation} satisfies \emph{monotonicity}, in the sense that for two given corresponding data sets $\mathcal{D}$ and $\mathcal{D}'$}, $\mathcal{D}' \subseteq \mathcal{D}$ \moh{implies that} the abstraction model $\mathcal{H}_{\mathcal{D}'}$ over-approximates the abstraction model $\mathcal{H}_\mathcal{D}$.
\end{proposition}
\begin{proof} \moh{Let $J$ and $J'$ be the set of indices corresponding to data pairs included in $\overline{\mathcal{D}}$ and $\overline{\mathcal{D}'}$ (constructed from $\mathcal{D}$ and $\mathcal{D}'$) and $\forall i \in \{1\dots m\}$, $\overline{f}^i(s)$ and  $\overline{f'}^i(s)$, and $\underline{f}^i(s)$ and $\underline{f'}^i(s)$ are upper and lower  abstraction functions returned by the abstraction models $\mathcal{H}_{\mathcal{D}}$ and $\mathcal{H}_{\mathcal{D}'}$, respectively.} Then, $\mathcal{D}' \subseteq \mathcal{D} \implies \overline{\mathcal{D}'} \subseteq \overline{\mathcal{D}} \implies J' \subseteq J \implies \overline{f}^i(s)=$ $ \min_{j,\ell \in J} ((\tilde{y}^o_{j+1, \ell})^{(i)}+L^{(i)}_p\|s-\tilde{s}^o_{j,\ell}\|_p+\varepsilon^{(i)}_{t}) \leq  \min_{j,\ell \in J'} ((\tilde{y}^o_{j+1,\ell})^{(i)}+L^{(i)}_p\|s-\tilde{s}^o_{j,\ell}\|_p+\varepsilon^{(i)}_{t})= \overline{f'}^i(s) \implies $ $\overline{f}(s) \leq \overline{f}'(s)$ \moh{, where the second inequality holds since the two optimization problems have the same objective functions, but the constraint set of the latter is a subset of the former. By a similar argument,} $\underline{f}(s) \geq \underline{f}'(s)$. \moh{It follows from these two results that} $\mathcal{H}_{\mathcal{D}'}$ over-approximates $\mathcal{H}_\mathcal{D}$.
\end{proof}
% In our framework, the Lipschitz constant is unknown and it could be lazily estimated from data by following \cite{}:
% \begin{align}
% L_p = \max_{i\neq j} \frac{|y^i -y^j|}{|s^i-s^j|_p}.
% \end{align}
% For the data set $\mathcal{D}=\{(\tilde{s}^i, \tilde{y}^i)|i=1,2 \cdots, N\}$ corrupted by bounded noise, the constant can be estimated with following equation:
% \begin{align} \label{estimateL}
% L_p = \max_{i\neq j} \frac{|y^i -y^j|-2\varepsilon_v}{|s_i-s_j|_p+2\varepsilon_w}.
% \end{align}
% To guarantee the $L_p$'s `quality' \moh{NEEDS MORE EXPLANATION}for a unknown function, we \moh{leverage} a classical result on PAC learning linear separators\cite{PAC}:
% \begin{definition}[Linear Separators] \label{def:linear} For $\Gamma \subset \mathbb{R} \times \mathbb{R}$, a linear separator is a pair $(a, b)\in \mathbb{R}^2$ such that
% \begin{align} \label{eq:linsep}
% \forall(x, y) \in \Gamma: \ x \leq ay +b.
% \end{align}
% \end{definition}
% To find some linear separators $(a, b)$ for $\Gamma$ by sampling points in $\Gamma$, we assume that points of $\Gamma$ can be drawn by some unknown distribution $Dist$. The error of a pair $(a, b)$ is defined to be $\texttt{err}_{Dist}(a,b)=Dist({(x,y)\in\Gamma|x>ay+b})$ where $Dist(X)$ is the measure of points that $(a,b)$ violates linear separator under distribution $Dist$. The algorithm to find $(a,b)$ is given by Algorithm \ref{Alg1}. Then the following result hold,
% \begin{algorithm}[b] 
% \SetAlgoLined\DontPrintSemicolon \small
% % \KwData{$\tt{Models} \  \mathit{\mathcal{G}_1 \ \dots \mathcal{G}_{N_f}}$, $\tt{Input\text{-}}\tt{Output} \ \tt{Sequence} =  \mathit{\{u_\ell, y_\ell\}_{\ell=0}^{\ell=k-1}}$} 
% \SetKwFunction{findmodel}{findPair}
% % \SetKwFunction{check}{checkValid}
% \SetKwProg{func}{function}{}{}
% \func{\findmodel{$\Gamma$, $Dist$, $N$}}
% {
%   % $\tt{valid} \leftarrow  \mathit{[N_f]} $\\
%   % \For{$i=1:N_f$} {
%   % Check Feasibility of Theorem \ref{theorem2} \\
%   % \If{infeasible} 
%   % {
%   %   Remove $i$ from $\tt{valid}$
%   %   }
%   % }
%   Draw $N$ pairs of data $(x_1, y_1), (x_2,y_2),\cdots,(x_N,y_N)$ from $\Gamma$ based on distribution $Dist$ \\
%   Find $(a,b)$ $s.t. \ x_i \leq ay_i +b \ \forall i \in \{1,2,\cdots, N\}$ \\
%   \KwRet{$(a,b)$}
% }
% % \func{\check{$\mathcal{G}, \{u_k, y_k\}_{k=0}^{k=t}$}}
% % {
% %   Refer to Theorem \ref{theorem2} for its description \\
% %   \KwRet{$\tt{ifValid}$}
% % }
%   \caption{\moh{Linear Separator}}%: find pair $(a,b)$}
%   \label{Alg1}
% \end{algorithm}\normalsize
% \begin{proposition} \cite{kearns1994introduction}
% Let $\epsilon, \delta \in \mathbb{R}^+$. If number of sampling points $N\geq\frac{1}{\epsilon}\ln\frac{1}{\delta}$, then, with probability $P \geq 1 - \delta$, Algorithm \ref{Alg1} finds pair $(a,b)$ such that $\texttt{err}_{Dist}(a,b)\leq\epsilon$.
% \end{proposition}
% \begin{proof}
% The detailed proof can be f\moh{ou}nd in \cite{fan2017d}.
% \end{proof}
% \moh{Considering} Definition \ref{def:linear}, \moh{it is easy to verify} that \eqref{estimateL} is a special case of the linear separator \moh{\eqref{eq:linsep}}, \moh{with} $b=0$. Thus, \moh{what \eqref{estimateL} returns is guaranteed with high probability to be the true} Lipschitz constant \moh{of the original unknown function.} %from Equation \eqref{estimateL} can be ensured to work for future abstraction with high probability.

\input{sec_result2}
% \subsection {\moh{Abstraction-Based} Model Invalidation}
% In \moh{order to solve} Problem \ref{problem2}, we will assume the following:
% \begin{assumption} \label{assumption1}
% The length-$T$ output trajectories are only consistent with one unknown model. Thus, we must have $\mathcal{B}^T(\mathcal{G}) \cap \mathcal{B}^T(\mathcal{G}') =\emptyset$, where $\mathcal{G}$ is original model and $\mathcal{G}'$ is the model to be invalidated.
% %There exist and only exist one valid model 
% %$\mathcal{G}_i$, i.e., $\mathcal{G}_j$. % in the system.
% \end{assumption}
% \moh{SOME JUSTIFICATION FOR ASSUMPTION}
%  % \begin{lemma} \label{lemma_formulation}
%  % Given the partition of the space, the piecewise constraint: $x_{k+1}\leq$
%  % \end{lemma}
 
%  \moh{We apply an} optimization-based model \moh{invalidation} approach to determine if the model is incompatible with the observed length-$T$ input-output trajectory. Since we assume that only one original unknown model can be consistent, with a sufficiently accurate abstraction, where enough data is sampled according to Proposition \ref{Abs}, we can also assume that the length-$T$ input-output trajectory is only compatible with the abstracted model. Using this fact, we propose the following model invalidation algorithm that (in)validates the abstraction model $\mathcal{H}_\ell$:

% % \vspace{-0.1cm}
%  Given an abstracted model $\mathcal{H}_\ell$ and a length-$T$ output sequence $\{y_k\}_{k=0}^{k=T-1}$, the model is invalidated if the following problem is infeasible:
%  \begin{subequations} \label{MI_o}
%  \begin{align} \tag{MI}
%  \nonumber & \hspace{-0.3cm} \text{Find} \ {x_k}, w_k, v_k, \ \forall  k  \in\mathbb{Z}_{T-1}^0         \\[-0.2em]
%  \nonumber &\hspace{-0.3cm} \text{subject to} \  \forall  k  \in\mathbb{Z}_{T-1}^{n_y-1}: \\
%  & \hspace{0.5cm} x_{k+1} \leq \overline{f}(s_k) + w_k\mathds{1}_n\label{constraint_1},\\[-0.2em]
%  & \hspace{0.5cm} x_{k+1} \geq \underline{f}(s_k) + w_k\mathds{1}_n,\label{constraint_2}\\[-0.2em]
%  % & \hspace{0.5cm} S_ix_k +T_iu_k\leq \beta_i + s_{i,k} \mathds{1}_{c_i}, \label{constraint_3}\\[-0.2em]
%   \nonumber & \hspace{0.5cm} \forall k \in \mathbb{Z}_{T-1}^0:  \\[-0.2em]
%   & \hspace{0.5cm} y_k = x_k+v_k, \ \underline{x}_k \leq x_k \leq \overline{x}_k,\\[-0.2em]
%   % & \hspace{0.5cm}   \\[-0.2em]
%   & \hspace{0.5cm} ||w_k||\leq \varepsilon_w, \ ||v_k||\leq \varepsilon_v,
%  % &\hspace{.5cm}  a_{i,k}\in\{0, 1\}, \ \textstyle\sum_{i\in[p]} a_{i,k}=1, \label{constraint_sos1}\\[-0.2em] 
%  % & \hspace{0.5cm} ||\omega_k||\leq \varepsilon_\omega, \ ||v_k||\leq \varepsilon_v, \ (a_{i,k}, s_{i,k}):SOS\text{-}1,
%  \end{align}
%  \end{subequations}
%  where $s_k=[x_k,\cdots,x_{k-n_y+1}]^T$, $\underline{x}_k$ and $\overline{x}_k$ are given bounds of $x_k$. \moh{Through the following Theorem \ref{theorem2}, we will show}
% \begin{theorem} \label{theorem2}
%  Solving problem (MI) is equivalent to check if the following problem is infeasible:
%  \begin{subequations}
%  \begin{align}
%  \nonumber & \hspace{-0.3cm} \text{Find} \ {x_k}, w_k, v_k, \ \forall  k  \in\mathbb{Z}_{T-1}^0         \\[-0.2em]
%  \nonumber &\hspace{-0.3cm} \text{subject to} \  \forall  k  \in\mathbb{Z}_{T-1}^{n_y-1}: \\
%  & \hspace{0.3cm} x_{k+1} \leq \tilde{y}^i+L_p|\tilde{s}^i-s_k|_p + w_k\mathds{1}_n,\ \forall (\tilde{s}^i,\tilde{y}^i)\in\mathcal{D} \\[-0.2em]
%  & \hspace{0.3cm} x_{k+1} \geq \tilde{y}^i+L_p|\tilde{s}^i-s_k|_p + w_k\mathds{1}_n,\ \forall (\tilde{s}^i,\tilde{y}^i)\in\mathcal{D} \label{constraint2'}\\[-0.2em]
%  % & \hspace{0.5cm} S_ix_k +T_iu_k\leq \beta_i + s_{i,k} \mathds{1}_{c_i}, \label{constraint_3}\\[-0.2em]
%   \nonumber & \hspace{0.3cm} \forall k \in \mathbb{Z}_{T-1}^0:  \\[-0.2em]
%   & \hspace{0.3cm} y_k = x_k+v_k, \ \underline{x}_k \leq x_k \leq \overline{x}_k, \\[-0.2em]
%   % & \hspace{0.3cm} \underline{x}_k \leq x_k \leq \overline{x}_k,  \\[-0.2em]
%   & \hspace{0.3cm} ||w_k||\leq \varepsilon_w, \ ||v_k||\leq \varepsilon_v,
%  % &\hspace{.5cm}  a_{i,k}\in\{0, 1\}, \ \textstyle\sum_{i\in[p]} a_{i,k}=1, \label{constraint_sos1}\\[-0.2em] 
%  % & \hspace{0.5cm} ||\omega_k||\leq \varepsilon_\omega, \ ||v_k||\leq \varepsilon_v, \ (a_{i,k}, s_{i,k}):SOS\text{-}1,
%  \end{align}
%  \end{subequations}
%  where $\mathcal{D} = \{(\tilde{s}^i, \tilde{y}^i)|i=1,2 \cdots, N\}$ is the given data set for model $\mathcal{H}_\ell$.
% \end{theorem}
% % \vspace{-0.35cm}
% \begin{proof}
% Since the upper bound of the abstraction is given by \eqref{upper_func}, constraint \eqref{constraint_1} is equivalent to $x_{k+1} \leq \tilde{y}^i+L_p|\tilde{s}^i-s_k|_p + w_k\mathds{1}_n,\ \forall (\tilde{s}^i,\tilde{y}^i)\in\mathcal{D}$. The \eqref{constraint2'} is equivalent to \eqref{constraint_2} for the same reason. Thus, two optimization problems are equivalent. If the above optimization problem (hence, \eqref{MI_o}) is infeasible, it means that the output sequence $\{y_k\}_{k=0}^{k=N-1}$ cannot be consistent with the length-$T$ behavior of $\mathcal{H}_\ell$, i.e., $\{y_k\}_{k=0}^{k=N-1} \notin \mathcal{B}^N(\mathcal{H}_\ell)$, hence the model is invalidated.
% \end{proof}
% According to Remark \ref{linear}, the optimization problem can be LP problem by choosing the suitable norm. Based on the Proposition \ref{Abs}, the computational time can be further reduced by picking points from original data set at the cost of the model precision. We will explore this in the simulation part.



